TwinTex: Geometry-aware Texture Generation for Abstracted 3D Architectural Models

Coarse architectural models are often generated at scales ranging from individual buildings to scenes for downstream applications such as Digital Twin City, Metaverse, LODs, etc. Such piece-wise planar models can be abstracted as twins from 3D dense reconstructions. However, these models typically lack realistic texture relative to the real building or scene, making them unsuitable for vivid display or direct reference. In this paper, we present TwinTex, the first automatic texture mapping framework to generate a photo-realistic texture for a piece-wise planar proxy. Our method addresses most challenges occurring in such twin texture generation. Specifically, for each primitive plane, we first select a small set of photos with greedy heuristics considering photometric quality, perspective quality and facade texture completeness. Then, different levels of line features (LoLs) are extracted from the set of selected photos to generate guidance for later steps. With LoLs, we employ optimization algorithms to align texture with geometry from local to global. Finally, we fine-tune a diffusion model with a multi-mask initialization component and a new dataset to inpaint the missing region. Experimental results on many buildings, indoor scenes and man-made objects of varying complexity demonstrate the generalization ability of our algorithm. Our approach surpasses state-of-the-art texture mapping methods in terms of high-fidelity quality and reaches a human-expert production level with much less effort. Project page: https://vcc.tech/research/2023/TwinTex.

==> src/backup/01-intro.tex <==
\section{Introduction}
\label{sec:intro}

\ignore{Automatic 3D reconstruction of large-scale urban environments has experienced an increasing interest in computer graphics and compute vision communities. With the advances in active sensors (\eg LiDAR) and fully automated \emph{Multiple View Stereo} (MVS), many mature algorithms have been developed to generate complete and high-fidelity 3D geometry models~\cite{musialski2013survey}. Especially the recent aerial-based photogrammetry sensing technology achieves the generation of city-scale surface models from aerial oblique images, which are also enriched with high resolution textures~\cite{Smith2018Aerial,Hepp2018Plan3D,DroneScan20}. %,Liu2021Aerial,zhang2021continuous}.
}

\ignore{Although yielding impressive 3D reconstruction, all of these methods generate triangular meshes containing a huge amount of details. Such a dense mesh is a very redundant 3D representation and also lacks high-level semantic and structural information. The direct use of such meshes is often intractable in practical applications, for example, causing a lot of burden on model storage, transmission, editing, and real-time rendering. Therefore, there is rising attention to transforming dense meshes into simplified and concise polygonal models by either geometry simplification/approximation~\cite{garland1997surface,cohen2004variational,salinas2015structure} or structure-aware surface reconstruction~\cite{verdie2015lod,kelly2017bigsur,bauchet2020kinetic,bouzas2020structure}. }


\ignore{We propose a framework to automatically generate realistic texture to coarse building models, commonly referred to as mass models. }

With the advances in active sensors (\eg LiDAR), fully automated \emph{Multiple View Stereo} (MVS) and aerial-based photogrammetry sensing technology, many mature algorithms have been developed to generate complete and high-fidelity 3D dense reconstruction~\cite{musialski2013survey,Smith2018Aerial,DroneScan20} with textures~\cite{waechter2014let}. Architectural models with simplified topology and twin shapes of such dense models can be generated from procedural modeling, approximated from dense reconstruction, or created manually by artists and architects. These abstracted twin models are tractable in plenty of downstream applications due to their sharper features, much lower needs on storage, \ignore{more intuitive in editing, }and more suitable for transmission and real-time rendering, as shown in Fig.~\ref{fig:abstraction}.


\begin{figure}[tbh!]
	\centering
	\includegraphics[width=\linewidth]{images/fig2.pdf}
	%\vspace{-7mm}
	\caption{Left: Aerial distribution of the drone that collected the input photos (559 images). Top right: 3D dense reconstruction of a Headquarter. Bottom right: An abstracted twin model with a much smoother appearance and smaller storage needs.}
	%\vspace{-4mm}
	\label{fig:abstraction}
\end{figure}


However, the texture information contained in the original dense reconstruction is often not maintained after abstraction. Thus, with all the calibrated RGB images, how to texture the twin proxy for the level of realism then becomes a challenging problem.
An intuitive way is to employ image-based texture generation methods ~\cite{lempitsky2007seamless,waechter2014let,zhou2014color}. However, these approaches would produce distorted and misaligned artifacts as illustrated in Fig.~\ref{fig:texturing-issues}.
Although patch-based optimization method~\cite{bi2017patch} can reduce such artifacts to some extent by synthesizing photometrically-consistent aligned images to correct misalignments, it would possibly deliver blurring textures or missing regions. These issues are mainly caused by: \romannumeral1) the inaccurate camera parameters, \romannumeral2) the significant geometric differences between the twin mesh and ground-truth models brought by the abstraction process, and \romannumeral3) the large difference among viewing angles. The combination of these cases makes our problem even more challenging and complicated.
\wdx{The urban proxy models often exhibit large-scale planar structures. In practice, the modeling artists often manually create high-quality textures plane-by-plane. }
%(as shown in Fig.~\ref{fig:texturing-methods}).
However, this is an extremely tedious, time-consuming, and labor-intensive process. It took quite a few days for a professional modeler to texture an abstracted model such as the Polytech shown in Fig.~\ref{fig:teaser} with real photos. Texturing a model with a higher level of detail would take much longer.

\ignore{For such planes, in the view selection step, previous approaches may not find a suitable image that contains all the texture information for a large triangular face, leading to this triangular face untextured.}


\ignore{\begin{figure}%[tbh!]
	\centering
	\includegraphics[width=\linewidth]{images/dense2abstract}
	%\vspace{-5mm}
	\caption{Texturing results on Highrise using three different methods. From left to right: A dense model reconstructed with RealityCapture (RC); An abstracted version textured with a face-based method, LTBC~\cite{waechter2014let}; And the abstracted version textured manually by a senior Technical Artist based on pieces of planes.}
	\label{fig:texturing-methods}
\end{figure}}

\begin{figure}%[tbh!]
	\centering
	\includegraphics[width=\linewidth]{images/issues}
	%\vspace{-3mm}
	\caption{Illustration of several typical issues occurred in texturing architectural proxies.}
	%\vspace{-3mm}
	\label{fig:texturing-issues}
\end{figure}

%A simplified version textured with Patch-Based Optimization algorithm (PBO)~\cite{bi2017patch};

In this paper, we propose a plane-based methodology and fully automated algorithms to generate high-quality texture maps for piece-wise planar architectural models given a large set of unordered RGB photos. Our method addresses most challenges occurring in such twin texture generation: the large number and high resolution of input images, their drastically varying properties such as photometric quality, perspective quality (large variation of viewing angles), heavy occludes (\eg trees and buildings), and texture-geometry misalignment (introduced by incorrect camera parameters and model abstraction process).
%\wdx{Our algorithm consists of three main steps: plane-oriented view selection, line-guided texture stitching and texture optimization.}
Given a coarse model, our algorithm decomposes it into a set of planar polygonal shapes, for each of which we aim at generating a high-quality and complete texture map. We first present a plane-oriented view selection approach to select views that best cover each planar shape with high photometric and perspective consistency. Based on the line segments extracted from each view, a line-guided texture stitching is introduced to create a single texture map to preserve geometric features. Finally, we perform texture optimization to improve the illumination consistency and fill the missing regions in the texture map.
Experiments are performed to show the effectiveness and robustness of our method.
In summary, our work makes the following contributions:
%The major contributions are concluded as follows:
\begin{itemize}
\item A fully automatic \textbf{TwinTex}, which produces high-quality and geometry-aware texture for a simplified proxy model.

\item A view selection algorithm that can select a small number of candidate photos for each primitive plane considering texture completeness, perspective and photometric quality.

\item A plane-based texture mapping methodology via geometry-aware image stitching guided by LoLs.

\item An architectural dataset including various scenes and building components. We utilize this dataset and fine-tune a diffusion probabilistic model with a novel multi-mask initialization component to complete the texture maps.

%\item \wdx{A multi-masks initialization component . An architectural dataset including various scenes and building components. We utilize this dataset and fine-tuned a diffusion probabilistic model to complete the texture maps.}
\end{itemize}








==> src/backup/02-rw.tex <==
\section{Related Work}\label{sec:rw}

\subsection{Image-based Texture Mapping}

Texture mapping is an important approach for authoring photo-realistic 3D objects without increasing their geometric complexity~\cite{yuksel2019rethinking}.
View-dependent texture mapping works~\cite{debevec1996modeling,debevec1998efficient} composite multiple views of a scene by assuming the existence of a global mesh and storing all appearance variation in textures.
\ignore{The final images can be interactively rendered with image-based rendering techniques to provide realistic imagery.}
%While producing realistic imagery from novel viewpoints,
Although they also use a view selection procedure to project a single image onto the model and then merge several image projections, they only determine for each polygon in the model in which photos it is visible.
\ignore{In addition, these methods do not produce a globally consistent texture map, limiting their applications in a new environment with different lighting conditions. }
Instead, we present a novel view selection algorithm that considers texture completeness, perspective quality, and photometric quality.
% Existing 3D reconstruction methods suffer from various inaccuracies, including missing or spurious additional geometry, misalignment between geometry and image boundaries, and excessively smooth or noisy geometry

To generate a single consistent texture map, early works on image-based texture mapping usually select multiple images for each face and blend them into textures by using different weighting strategies~\cite{bernardini2001high, callieri2008masked}. However, such methods could generate blurry and ghosting results due to camera calibration errors and inaccurate geometry.
To reduce those artifacts caused by multi-image blending, later approaches choose to select only one view per face, then conduct seam optimization to create a texture patch and to avoid visible seams between adjacent patches~\cite{lempitsky2007seamless,wang2018seamless,gal2010seamless, waechter2014let,fu2018texture,fu2020joint}. They typically solve a discrete labeling problem by using different data terms and smoothness terms to construct the Markov random field to select an optimal  texture image for each face.
Whereas, \ignore{as shown in Fig.~\ref{fig:texturing-issues}, }these approaches still suffer from misaligned seams in challenging cases.
Another category of warping-based methods jointly rectifies the camera poses and geometric errors. Zhou and Koltun~\shortcite{zhou2014color} use local image warping to optimize camera poses in tandem with non-rigid correction functions for all images. This approach is then extended by~\cite{bi2017patch} to propose a patch-based optimization that handles larger geometry inaccuracies by correctly aligning the input images. This method estimates the bidirectional similarity of different images, which suffers from high computational costs.



\ignore{However, all the above methods directly map the color information of high-resolution images to the 3D reconstructed mesh.}

Although high-quality texture maps can be generated from the above methods, the resultant quality of texture mapping still greatly depends on the quality of reconstruction and accuracy of camera calibration. None of them can be naively applied to generate the realistic texture of a large-scale structured building or scene. Firstly, the abstracted proxy model has significant structural differences from the original dense mesh. Moreover, constrained by the complicated environment, the collected aerial data often has highly uneven camera distribution, large camera calibration errors and large variations in viewing angles. Current methods still cannot handle these problems well, resulting in obvious artifacts. Instead, we choose to generate texture in a plane-based manner that is more intuitive and human alike.


\begin{figure*}[tp]
	\centering
	\includegraphics[width=\linewidth]{images/fig4-pipeline.jpg}
    %\vspace{-0.6cm}
	\caption{Overview of our algorithm on the Hitech building. Taking an abstracted model and the UAV images as input, our framework detects the proxy polygons in the mesh and generates one stitched texture map for each proxy polygon. Firstly, a small subset of views is selected from all the visible views for each proxy polygon. Then, all the selected views are stitched together to form an enlarged texture map. Note that important geometric primitives such as line segments contained in the original images are well preserved after the image stitching. Finally, the texture map is optimized by performing global consistency across all the visible regions and inpainting the incomplete region of the underlying planar shape.}
	\label{fig:pipeline}
\end{figure*}

% Although high-quality texture maps can be generated from above methods,
% easily computed for accurate geometry and calibrated cameras, the quality of texture map degrades signifcantly in the presence of inaccuracies.

\subsection{Structure-aware Scene Reconstruction and Texturing}

Creating structured models from noisy raw data has become an ever-increasing demand in urban digitization. \jw{\citet{ceylan2012factored,ceylan2014coupled} propose image-based 3D urban building reconstruction frameworks by exploiting the presence of linear and symmetric features (\eg lines, repeated elements) in facade for image registration and 3D reconstruction.
To generate simplified meshes,} a popular way is to first reconstruct a 3D dense mesh and then simplify it using geometry simplification~\cite{garland1997surface} or piece-wise planar structure approximation methods~\cite{cohen2004variational, verdie2015lod, salinas2015structure}. Another way is to directly detect a set of planar primitives from the point clouds, then explore the arrangements of primitives to provide a compact polygonal mesh~\cite{Monszpart2015rapter, Nan2017polyfit, fang2020connect, bauchet2020kinetic, bouzas2020structure, Pan2022Efficient, Guo2022}. In practice, such proxy models are usually generated manually or by procedural modeling~\cite{sinha2008interactive} with arbitrary topology (\eg manifolds or non-manifolds).

\ignore{In our approach, we utilize an efficient and robust structure-aware surface reconstruction~\cite{Pan2022Efficient} to generate simplified meshes from point clouds or raw triangular meshes.}

However, texturing such abstracted building models has drawn less attention. Several methods take into account the generation of texture maps while conducting a lightweight geometric reconstruction~\cite{sinha2008interactive, garcia2013automatic, huang20173dlite, maier2017intrinsic3d, wang2018plane}. For example, \citet{garcia2013automatic} computes a per-building volumetric proxy, then uses a surface graph-cut method to stitch aerial images and yield a visually coherent texture map. However, their reconstruction results are 2.5D which can only restore textures under limited perspectives, losing important structures.
%\ignore{Aiming at indoor scene reconstruction, 3DLite~\cite{huang20173dlite} presents a primitive-based scene abstraction, then uses the planar-based constraint to generate high-quality textures on abstracted geometry through texture optimization.Due to a lot of assumptions on the structure of the indoor scenes and too many texture loss functions to be optimized, the generalization of this method is limited and its convergence speed is pretty slow.}
Recently, deep learning approaches based on image-image translation networks have been proposed to synthesize texture details for coarse meshes of urban areas~\cite{Kelly2018FrankenGAN, georgiou2021projective}. Although data-driven methods are able to generate various styles of textures, they require extensive training sets, and the synthesized textures lack realism comparing to the original real scenes.
The technique of NeRF~\cite{mueller2022instant} shows great ability to generate high-quality 3D shapes and textures~\cite{metzer2022latent,baatz2022nerf}. However, remember that we aim at very high-resolution input and output images which require extremely large memory, employing a small set of input images is not enough for NeRF-based methods to generate satisfying results, which makes them less applicable in our scenario. %We suggest readers check our supplemental for the details on input images.

\subsection{Image Stitching and Completion}

Image stitching is to combine multiple images with overlapping sections to produce a single panoramic or high-resolution image~\cite{szeliski2007image, Mehta2011}.
%is a central and long-studied problem in computer graphics~\cite{szeliski2007image,Mehta2011}.
Early methods estimate an optimal global transformation for each input image~\cite{brown2007automatic}. However, they only work well for scenes near planar or with slight view disparity, and usually generate ghosting artifacts or projective distortion for general scenes.
For more accurate stitching, many approaches adopt spatially-varying warps to process different regions of an image, including smoothly varying affine transformation~\cite{lin2011smoothly}, dual or quasi homographies~\cite{gao2011constructing, li2017quasi}, shape-preserving half-projective warps~\cite{chang2014shape, lin2015adaptive}, and smoothly varying homography field~\cite{zaragoza2013projective}, etc.
\jw{Aiming at building facades, \citet{musialski2010interactive} present a system for generating approximately orthographic facade textures from a set of perspective photographs. They perform multi-view image stitching over planar proxies by using a gradient-domain stitching to avoid visible seams.}

However, they are usually time-consuming and unsuitable for scenes with large parallax and view disparity. Several methods are then proposed to obtain better alignment with less distortion, especially for large parallax~\cite{zhang2016multi, lee2020warping}, but linear structures in the image are not well maintained. After that, instead of just using point feature matching, line features are introduced to preserve both linear structures~\cite{li2015dual, xiang2018image, liao2019single, jia2021leveraging}.
All these methods apply a uniform grid to warp the images, which are not flexible enough to align the regions with dense geometric features. Unlike them, we propose to use an adaptive grid to locally warp the images and better align the large-scale line features.

%WD: not sure how this step would go, will change later, introduce diffusion model, the Repaint.

Image completion, also known as image inpainting, is the process of restoring missing or damaged areas in an image. Extensive research has been conducted on image completion, and existing methods can be classified into three types: 1) diffusion-based methods, 2) patch-based methods and 3) deep learning methods based on generative models. A detailed review is out of the scope of this paper, and we refer the reader to recent works~\cite{dhariwal2021diffusion, lugmayr2022repaint} and surveys~\cite{guillemot2014image, rojas2020a, elharrouss2020image, jam2021a}.



==> src/backup/03-overview.tex <==
\section{Problem Statement and Overview}
\label{sec:overview}

The objective of our approach is to automatically generate realistic and geometry-aware texture maps for a piece-wise planar model, \ie urban building or scene.
Our algorithm takes a set of calibrated camera views $\{ \mathcal{I} \}$ and an abstracted model $\mathcal{M}$ as input, and outputs high-quality texture maps. 
%To be precise, the tuple of $\mathcal{(I, T, K)}$ represents the collected images, and extrinsic and intrinsic camera parameters \jwc{if we mention the extrinsic and intrinsic camera parameters in later? if not, this sentence can be deleted}. %$\mathcal{M}$ is a polygonal mesh where each basic element of $\mathcal{E}$ is an edge and $\mathcal{F}$ is either a polygonal or triangular facet.
The proxy model $\mathcal{M}$ is a polygonal mesh consisting of a set of planar polygonal shapes $\mathcal{P}_i$, each of which is referred to as a \emph{proxy polygon}.

\ignore{~\cite{verdie2015lod, kelly2017bigsur, fang2020connect, bauchet2020kinetic, bouzas2020structure}.}
%$\mathcal{M=(E, F)}$

%After obtaining primitive polygons $\{\mathcal{M}_i\}$,
To produce a texture map for each proxy polygon $\mathcal{P}_i$, the first step should be to select one or multiple images as candidate maps for $\mathcal{P}_i$. However, unlike previous texturing problems dealing with dense models (small triangles), it is usual that none of the given images can cover such large proxy polygons in abstracted versions. Hence, we employ the latter scheme and select multiple images for each polygon shape.
However, there are still several challenges that exist in our scenario: i) Photometric issue. There are seams, illumination resolution inconsistency between adjacent patches. For large scale scenes, the frequent ghosting effect is mainly introduced by the dynamic instances, such as cars and tower crane. ii) Perspective issue. Even with photometric consistent patches, it would still be apparent that the stitched texture comes from several images with largely varied viewing angles. iii) Image-to-image and image-to-geometry misalignment. This is introduced by both the inaccuracy of camera parameters and the simplification process. iv) Facade incompleteness. In the absence of semantic guidance, how to fill a largely empty region with geometrically and semantically consistent content remains a problem.

\ignore{However, the city building textures are far more complicated and sometimes hard to represent by an existing label of components. }

\ignore{\begin{figure}[!tbh]
	\centering
	\includegraphics[width=.8\linewidth]{images/plane_extraction.pdf}
  	%\vspace{-3mm}
	\caption{All facets of input mesh $\mathcal{M}$ is first segmented into a set of planar regions represented with proxy polygons $\{\mathcal{P}_i\}$. The shape of each proxy polygon is then extracted as proxy boundary $\mathcal{B}_i$ (visualized with red border lines).}
	%\vspace{-3mm}
	\label{fig:boundary_extraction}
\end{figure}}

\begin{figure}[!tbh]
	\centering
	\includegraphics[width=.75\linewidth]{images/plane_extraction.pdf}
	%\vspace{-3mm}
	\caption{The input mesh $\mathcal{M}$ is first segmented into a set of planar regions represented with proxy polygons $\{\mathcal{P}_i\}$. The shape of each proxy polygon is then extracted as proxy boundary $\mathcal{B}_i$ (visualized with red border lines).}
	%\vspace{-3mm}
	\label{fig:boundary_extraction}
\end{figure}


To address the above problems, we propose a plane-based and geometry-aware texture mapping methodology, as shown in Fig.~\ref{fig:pipeline}.
First, we extract high-quality views and visible regions for each proxy polygon $\mathcal{P}_i$. An effective greedy heuristic method is proposed to select a small set of views $\{\mathcal{I}\}_i$ that best cover each $\mathcal{P}_i$ with high photometric and perspective consistency (Sec.~\ref{sec:view-selection}).
Next, in Sec.~\ref{sec:LOLs}, the rich line features contained in the selected images $\{\mathcal{I}\}_i$ are detected and organized into Level of Lines (LoLs).
After that, all the selected images are sequentially warped to their relative proxy boundary based on LoLs and stitched into a single texture map. Sec.~\ref{sec:texture-stitching} provides details.
Then, each texture map is optimized by a series of operators to reveal illumination consistency. Finally, we provide an architectural image dataset and train a multi-mask Diffusion Model to inpaint the missing regions in texture maps, see Sec.~\ref{sec:texture-optimization}.
% Experiments are performed to show the effectiveness and feasibility of our framework in Sec.~\ref{sec:results}.
Our algorithm has been implemented as a customized plug-in of a widely used graphics engine called Houdini\footnote{https://www.sidefx.com/}.

%User studies with in-field TAs are carried out to show the usability of our tool \red{in Sec.~\ref{sec:user-study}}.



% Such a piece-wise planar mass model can be considered as an assembly of planar polygonal shapes. In this manuscript, we represent each shape as a \textbf{proxy polygon}, $\mathcal{M}_i \subset \mathcal{M}$, consisting of faces. We extract $\mathcal{M}_i$ by utilizing a region-growing algorithm based on face normal. We then detect the corresponding \textbf{proxy boundary} $\mathcal{B}_i$ by choosing and sorting the boundary edges of $\mathcal{M}_i$. Fig.~\ref{fig:boundary_extraction} shows the result of this step on a Science Building.

% organize the key problems we need to handle and how we do that.


\ignore{Directly applying previous methods to select the best view for each facet can not guarantee that most part of each planar region is textured by only a few image patches. Moreover, visible seams occurring at the boundary of adjacent patches would damage the visual quality of generated texture.}

% needs a figure here to visualize those issues

\ignore{key problems we need to solve using the plane-based texturing heuristic:
	\begin{itemize}
		\item possibly no single photo can cover a big plane, need to merge multiple images into one to cover as much plane area as possible, hence could possibly generate lots of obvious visual artifacts such as seams, photometric inconsistency, resolution inconsistency and incompleteness. These are traditional texturing mapping problems.
		\item especially, representing a building facet with multiple photos would face a perspective problem in that the viewing angles may heavily vary from each other. So how to select candidate key views with high perspective consistency remains a problem.
		\item the inconsistency between texture and geometry. This is introduced by both the inaccuracy of camera parameters and the simplification process. These two factors jointly make inconsistency a heavier problem.
		\item semantic facade texture inpainting. traditional facade inpainting relies on semantic layout structural info as input. However. The city building textures are far more complicated and sometimes hard to represent by simple facade components. How to fill the empty region in a facade with geometrically and semantically consistent content in a more flexible way.
\end{itemize}}


% kind of feel that "target image" is not a good name, change it to "source image", and reference image to "proxy boundary"


% In this manuscript, we propose a plane-based and geometry-aware texture mapping methodology to address most of the above problems. Our method mainly consists of three parts: plane-oriented view selection, line-guided texture mapping and inpainting. Fig.~\ref{fig:pipeline} illustrates the pipeline of our algorithm.
% First, we extract high-quality views and visible regions for each proxy polygon $\mathcal{P}_i$. In Sec.~\ref{sec:view-selection}, an effective greedy heuristic method is proposed to select a small set of views $\{\mathcal{I}\}_i$ that best cover each $\mathcal{P}_i$ with high photometric and perceptual consistency.
% Next, in Sec.~\ref{sec:LOLs}, the rich line features contained in the selected images $\{\mathcal{I}\}_i$ are detected and organized into Level of Lines (LoLs). After that, in Sec.~\ref{sec:texture-optimization}, all the selected images are sequentially warped to their relative proxy boundary $\mathcal{B}_i$ based on LoLs. Then, each texture map is optimized by a series of operators to reveal global photometric consistency.
% Finally, in Sec.~\ref{sec:texture-inpainting}, we introduce a Line-guided probabilistic Diffusion Model (LDM) to inpaint all the missing regions in texture maps.
% Experiments are performed to show the effectiveness and feasibility of our framework in Sec.~\ref{sec:results}. Furthermore, our methods are implemented as a customized plug-in of a widely used graphics engine called Houdini. User studies with in-field TAs are carried out to show the usability of our tool in Sec.~\ref{sec:user-study}.




==> src/backup/04-selection.tex <==
\section{Plane-oriented View Selection}
\label{sec:view-selection}

%The variance of photo quality, position and the inaccuracy of camera/geometry will all magnify the problem of photometric and perceptual inconsistency, generating obvious seams/cracks, misalignment or blurring effects.

\paragraph{Proxy polygon extraction.}
The input proxy $\mathcal{M=(E, F)}$ can be created manually, generated procedurally, or abstracted from a dense reconstruction. %~\cite{kelly2017bigsur,bauchet2020kinetic}.
$\mathcal{M}$ is a polygonal mesh where each basic element of $\mathcal{E}$ is an edge and $\mathcal{F}$ is either a polygonal or triangular facet, as shown in Fig.~\ref{fig:boundary_extraction}. We first segment $\mathcal{M}$ into a set of planar polygonal shapes, each of which is represented as a \emph{proxy polygon} $\mathcal{P}_i$. We input $\mathcal{P}_i$ by utilizing a region-growing algorithm based on face normal. We then detect the corresponding proxy boundary $\mathcal{B}_i$ by choosing and sorting the boundary edges of $\mathcal{P}_i$. Fig.~\ref{fig:boundary_extraction} shows the result of this step on the scene of Hitech.

\textbf{View selection.}
Given a large set of input calibrated photos, the goal of this step is to select a small set of camera views ${ \{ \mathcal{I} \} }_{i}$ as candidate feature maps to best cover each proxy polygon $\mathcal{P}_i$.
We first apply frustum-culling and visibility detection to filter out the views and pixels which are invisible, far away from $\mathcal{P}_i$, or have extremely inclined viewing angles. The filtered images are then projected onto $\mathcal{P}_i$, and the projected regions $\{ \mathcal{R} \}$ covering the proxy polygon are extracted as candidate images, as shown in Fig.~\ref{fig:pipeline}.

\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{images/view_selection.pdf}
	%\vspace{-0.5cm}
	\caption{The view selection process of a proxy polygon $\mathcal{P}_i$. The red polygons denote the observed regions, while the grey ones denote the unobserved regions. The polygon with blue outline denotes the incremental region ${A_i^j}$ of selected image $\mathcal{R}_{j}$ in the current iteration. }
	%\vspace{-4mm}
	\label{fig:selection}
\end{figure}

\ignore{\begin{figure}[tbh]
		\centering
		\includegraphics[width=\linewidth]{images/projection.png}
		%\vspace{-2mm}
		\caption{Projection of a filtered image to the target proxy polygon. \wdx{the image before and after projection is not the same one. need to update}}
		\label{fig:projection}
\end{figure}}

After that, we propose an iterative view selection algorithm to select a smaller set of candidate views from the projected images covering $\mathcal{P}_i$ (see Fig.~\ref{fig:selection}).
%In the beginning, the set of selected candidate images is empty, i.e., $\{ \mathcal{I} \}_{i}^{0}=\emptyset$. In iteration $k$, the ${\mathcal{R}_j}$ with the highest quality (denoted by $Q_j$) is picked up and we create $\{ \mathcal{I} \}_{i}^{k} = \{ \mathcal{I} \}_{i}^{k-1} \cup R_j$.
%%put into $\{ \mathcal{I} \}_{i}^{k-1}$.
Starting from an empty set $\{\mathcal{I} \}_{i}^{0}=\emptyset$, we select the best projected image ${\mathcal{R}_j}$ with the highest quality (denoted by $Q_j$) in each iteration $k$ to create $\{ \mathcal{I} \}_{i}^{k} = \{ \mathcal{I} \}_{i}^{k-1} \cup R_j$.
This process converges when there is no projected image left to examine, or the $\{ \mathcal{I} \}_{i}^{k}$ can fully cover $\mathcal{P}_i$, i.e., the area of unobserved regions in $\mathcal{P}_i$ is smaller than a given threshold $\tau$.
We measure the quality $Q_j$ of each ${\mathcal{R}_j}$ by its incremental coverage ratio of the proxy polygon, its photometric and perspective quality and consistency with $\{\mathcal{I} \}_{i}^{k-1}$.
Specifically, the score $Q_j$ is calculated as the weighted sum of two terms:
\begin{equation}
	Q_j = Q_{photo} + {\lambda}_p Q_{persp} ,
\end{equation}
where $Q_{photo}$ and $Q_{persp}$ represent the photometric and perspective quality, respectively. $\lambda_p$ is the weight of $Q_{persp}$. %In the following paragraphs, we present the details of each term.
% The quality measurement of projected image $\mathcal{R}_j$ given $\{ \mathcal{I} \}_{i}^{k}$ mainly consists of two terms.

\paragraph{Photometric quality.} This term favors $\mathcal{R}_{j}$ with large incremental projection region, high resolution, and high photometric similarity to all the projected images and previously selected images. In detail, the coverage ratio of $\mathcal{R}_{j}$ against proxy polygon $\mathcal{P}_i$ at iteration $k$ is calculated as ${A_i^j}$/${{A_i}^k}$. It is determined by the area of the incremental region ${A_i^j}$ normalized with the unobserved area ${A_i}^k$.
\jw{Second, we measure the resolution of $\mathcal{R}_{j}$ as $G(\mathcal{R}_{j})$ by computing the average of the gradient magnitude over all pixels within the projection region~\cite{gal2010seamless}.} %normalized with 255.}
The photometric similarity, $C(\mathcal{R}_{j},\{ \mathcal{R} \})$, is defined by checking the photo-consistency of $\mathcal{R}_{j}$ against all the other projected images. It is computed by a multi-variate Gaussian function~\cite{waechter2014let}.
Furthermore, we introduce a new smoothness term to give a more confident value to a projected image $\mathcal{R}_j$ when $\mathcal{R}_j$ is consistent with the current set of selected images $\{\mathcal{I} \}_{i}^{k-1}$.
To sum up, the final photometric quality term is organized as:
\begin{align}
&Q_{photo} =  [ \lambda_g G(\mathcal{R}_j) + \lambda_c C(\mathcal{R}_j,\{\mathcal{R}\}) ] \dfrac{A_i^j}{{A_i}^k} + \lambda_s Q_{smooth} ,\\
&Q_{smooth} = 1 - D_c (\mathcal{R}_j, \{\mathcal{I} \}_{i}^{k-1}) ,
\end{align}
where $\lambda_g$ and $\lambda_c$ are the respective weight of $G(\mathcal{R}_j)$ and $C(\mathcal{R}_j,\{ \mathcal{R} \})$, $\lambda_s$ is the weight of $Q_{smooth}$. \hq{$D_c (\mathcal{R}_j, \{\mathcal{I} \}_{i}^{k-1})$ represents the mean of pixel-wise color difference} between the overlapping pixels of image $\mathcal{R}_j$ and all the images in $\{ \mathcal{I} \}_{i}^{k-1}$ after normalization. $Q_{smooth}=1$ if iteration $k$ is zero or there exists no overlapping regions. The quality term $Q_{photo}$ tends to select a set of projected images with the maximum photometric and content consistency, which helps reducing the ghosting effect.
\wdx{Note that both photometric and smoothness terms consider overlap regions. $C( \cdot )$ directly uses the whole projected regions (including overlap regions) of all the projected images $R$. Meanwhile, the smoothness term only considers the overlap region compared to the candidate projected image $I$.}

\paragraph{Pespective quality.} However, only considering the photometric quality will possibly cause significant perspective inconsistency among selected regions/patches. An example is shown at the bottom left in Fig.~\ref{fig:texturing-issues}, where the partial region is from the left viewing angles and the other regions come from the right viewing angles. %This can be observed in Fig.~\ref{fig:percep-b}.
One solution is to evaluate one patch at a time and choose patches with viewing directions as close to the normal of the current proxy polygon as possible~\hq{\cite{wang2018seamless}}.
However, the set of candidate photos usually has a large variation in viewing direction and extremely uneven distribution, especially for those proxy polygons with large planes.
Strong front-parallel constraint could introduce missing regions while loose constraint could cause significant perspective differences.
%We may never find applicable candidates with such a strong front-parallel constraint as previous work, which results in large missing regions.
To address this issue, we present a novel quality measurement to select a set of perspective consistent images, while satisfying the front-parallel constraint as much as possible.


The perspective quality term tends to select the next candidate image with a viewing direction similar to selected images in $\{ \mathcal{I} \}_{i}^{k-1}$, and with a viewing angle perpendicular to $\mathcal{P}_i$ as much as possible.
Hence, the perspective property is measured with front-parallel constraint and viewing angle consistency against selected photos. Unlike previous methods that only consider the viewing angle of a single candidate at a time~\hq{\cite{wang2018seamless}}, we propose to select a set of candidate images with high viewing angle consistency and as many front-parallel properties.
\wdx{Photo collections usually have a large variety of viewing angles. In practice, it is difficult to find a set of $N$ photos from the input all with a high level of front-parallelism covering a large plane. Compared to focusing on front-parallelism, we hope to stress more on viewing direction consistency as $N$ gets larger. Hence, we introduce the inverse facade normal as the first selected viewing direction.}
We define the perspective quality as:
%\vspace{-2mm}
\begin{equation}
Q_{persp}  = 1 - \dfrac{1}{N+1} [ D_{\hq{n}} (\mathbf{v}_j, -\mathbf{n}_i) + \sum_{n} D_{\theta} (\mathbf{v}_j, \mathbf{v}_n) ] ,
\end{equation}
where $N$ is the number of selected images in $\{ \mathcal{I} \}_{i}^{k-1}$, $\mathbf{n_i}$ is the plane normal of $\mathcal{P}_i$, $\mathbf{v}_j$ is the viewing direction of $R_j$, $\mathbf{v}_n$ is the viewing direction of the $n$-th image in $\{ \mathcal{I} \}_{i}^{k-1}$. \hq{$D_{n} (\mathbf{v},\mathbf{n}) = \frac{2}{\pi} \cos^{-1}{( \mathbf{v} \cdot \mathbf{n} )}$ calculates the normalized angular distance between facet normal $\mathbf{v}$ and plane normal $\mathbf{n}$.} $D_{\theta} (\mathbf{u}_1,\mathbf{u}_2) = \frac{\hq{1}}{\pi} \cos^{-1}{( \mathbf{u}_1 \cdot \mathbf{u}_2 )}$ calculates the normalized angular distance between facet normal $\mathbf{u}_1$ and $\mathbf{u}_2$.


% To sum up, the score $Q_j$ of a candidate image $\mathcal{R}_j$ is calculated as the weighted sum of the terms mentioned above:
% \begin{equation}
% 	Q_j = Q_{photo} + {\lambda}_p Q_{percep} ,
% \end{equation}
% where $\lambda_p$ is the weight of $Q_{percep}$. At iteration $k+1$, our greedy algorithm will select the image $\mathcal{R}_j$ with the largest value of quality $Q_j$, then create $\{ \mathcal{I} \}_{i}^{k+1} = \{ \mathcal{I} \}_{i}^{k} \cup R_j$. This process will repeat until the revealing area of $\mathcal{P}_i$ is smaller than a given threshold $\tau$.




==> src/backup/05-mapping.tex <==
%In this section, we present in detail three main phases involved in our plane-based texture generation approach.

%Directly apply previous triangular-facet based texture mapping methods to such data leads to inevitable mistakes as shown in Figure \ref{}. Thus, we proposed a plane-based texture mapping approach to handle those issues.

%In this section, we describe our texture mapping method based on planar structure for large-scale urban building. We extract planes and polygons from structured mesh (Section 4.1). These geometry structures will be used as the basic unit in view selection stage (Section 4.2). Finally a line preserved image stitching method will combine the patches from different views into a complete texture for each plane.


\section{Line-guided Texture Mapping}
\label{sec:texture-mapping}

After determining a set of high-quality images ${ \{ \mathcal{I} \} }_{i}$ for each proxy polygon $\mathcal{P}_i$, our next goal is to generate a realistic and geometry-aware texture map for $\mathcal{P}_i$.
Urban buildings usually exhibit rich structural information, such as local/global line features (e.g., window border/windows layout) in facades, and structural line features of the overall building (e.g., facade border). Different from most existing texturing methods that are dealing with overall smooth models, the proxy model in our case is only $C0$ continuous with obvious sharp structural features. It makes our texture mapping a challenging problem. Even tiny texture-to-texture or texture-to-geometry misalignments will draw great visual attention, which can be observed in Fig.~\ref{fig:misalignment}.
%One solution is to generate virtual textures based on semantic masks with labels of architectural components~\cite{Kelly2018FrankenGAN}. However, this method does not focus on the mapping of twin textures to real-world architecture. The generated styles of texture and categories of components are also limited by the training data.
%Another way is to interactively align those structural features~\cite {sinha2008interactive}, which is extremely labor-intensive and time-consuming for complex textures and mass models.

%The reasons are: i) even tiny misalignment between texture and geometry will draw great visual attention (i.e., misalignment between facade border in the texture map and facade boundary in planar polygon); ii) it is easy to notice the outliers among those line features with a high level of regularity.

\begin{figure}[!t]
	\centering
	\includegraphics[width=.9\linewidth]{images/misalignments.jpg}
	%\vspace{-0.3cm}
	\caption{Simply stitching selected images and projecting to proxy polygon produces obvious geometric inconsistency. Left: global texture-to-geometry misalignment, where the magenta textural feature lines should match the proxy geometric boundary (visualized in dark red). Right: local texture-to-texture misalignment, where the blue feature lines should be connected and collinear.}
	%\vspace{-4mm}
	%	\caption{Simply stitching selected images and projecting to proxy polygon produces obvious geometric inconsistency. The proxy boundary is visualized in dark red. Left: global texture-to-geometry misalignment, where the pink textural feature lines should match the red geometric borderline. Right: local texture-to-texture misalignment, where the orange feature lines should be connected and collinear.}
	\label{fig:misalignment}
\end{figure}


Instead of relying on semantic label masks to synthesize textures~\cite {sinha2008interactive}, we make full use of the rich line features extracted from candidate views and the proxy boundary extracted from the planar polygon to guide the texture mapping.
Our algorithm begins by extracting three levels of line features (LoLs) from selected candidate images. A line-guided texture stitching approach is then proposed to improve the visual effects based on LoLs. Finally, we perform a texture optimization step to further improve the illumination consistency and texture completeness.
To further eliminate the seams across patches, we employ graph-cut image synthesis~\cite{kwatra2003graphcut, boykov2001fast} and Poisson-Image-Editing~\cite{perez2003poisson} to obtain one single enlarged texture\ignore{by stitching visible regions and optimizing the blended textures} for each proxy polygon.

% Instead of relying on semantic label masks or manual works in texturing architectural mass, we choose to make use of the rich line features extracted from candidate views and the proxy boundary extracted from the planar polygon to guide the texture mapping.
% mainly consists of three phases. We first introduce the definition and extraction of LoLs from selected images in Sec.~\ref{sec:LOLs}. Next, in Sec.~\ref{sec:texture-stitching}, a line-guided texture stitching framework is proposed to improve the visual effect based on LoLs. Finally, a texture optimizaiton pipeline is introduced to further improve the illumination consistency and texture completeness in Sec.~\ref{sec:texture-optimization}. Finally, we employ graphcut image synthesis~\cite{kwatra2003graphcut, boykov2001fast} and Poisson-Image-Editing~\cite{perez2003poisson} approaches to eliminate the seams across patches. With this step, we obtain one single enlarged image by stitching each visible region and optimizing the blended texture for each proxy polygon.
%We will present the details of each sub-step in the remaining section.


\subsection{Levels of Line Features}
\label{sec:LOLs}

%Each step require line segments at different scales.
To generate proper line guidance at different scales we extract and optimize line segments from the level of local to global and finally define three levels of line features (LoLs). %In the following paragraphs, we will introduce the line extraction, refinement and matching processes.

\paragraph{$LoL_0$.}
We first employ the ELSED algorithm~\cite{suarez2022elsed} to detect rich but discrete line segments from the projected images $\mathcal{R}$ as local features at the finest scale.
%These line segments contain rich but discrete geometric line features without clear semantic meanings.
Then we organize these line segments into a set of global lines defined as $LoL_0$, in which each basic element encodes a meaningful primitive, \eg facade boundary, window boundary.
%Then we use a prominent structure-preserving algorithm~\cite{jia2021leveraging} to organize these line segments into a set of global lines defined as $LoL_0$, in which each basic element encodes a meaningful primitive, \eg facade boundary, window boundary.
The $LoL_0$ is employed for rigid registration (the details will be described in sec.~\ref{sec:texture-stitching}).
The registered images are then fed to later steps for generating $LoL_1$ and $LoL_2$.
% with higher accuracy


\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{images/LOLS}
	%\vspace{-0.6cm}
	\caption{\wdx{Three levels of the line features extracted from a facade image from local to global (left to right). The respective proxy boundary is visualized in red. Some refinement operations i)-iv) on $LoL_1$ are pointed with arrows.}}
	\label{fig:LoLs}
\end{figure}



\paragraph{$LoL_1$.}
%\wdx{With a registered image $\mathcal{I}_n$, we refine $LoL_0$ based on the proxy boundary $\mathcal{B}_i$ to generate $LoL_1$ containing global line elements matching the planar boundary.
\wdx{After registering image $\mathcal{I}_n$ via rigid alignment, we obtain its $LoL_1$ which has higher accuracy than $LoL_0$. However, the registered line segments still cannot well represent the polygon boundary. Our next step is to obtain $LoL_1$ which can maximally match $\mathcal{B}_i$.}

\wdx{We first measure the partial matching relationship of a line segment ${L} \in LoL_1$ compared to a boundary edge $b_m \in \mathcal{B}_i$ considering:}
a) $\theta({L},b_m)$, the angle between two lines.
b) $D_{l}({L},b_m)$, the maximum point-to-line distance from end-points to another line.
Moreover, it is useful in matching line segments with similar slopes and spatial distance, but large variances in length.
c) $N({L},b_m)$, the level of non-overlap between ${L}$ and $b_m$. To compute it, ${L}$ is first projected to $b_m$ to get ${L}^{'}$.
\wdx{We compute $N({L},b_m)$ based on four types of relationship between ${L}^{'}$ and $b_m$ after line projection, see the inset figure.}
\begin{wrapfigure}{r}{0.35\linewidth}
	\centering
	\includegraphics[width=\linewidth]{images/nonoverlap-inset}
\end{wrapfigure}
\wdx{In case 1 and 2, we assign infinity to $N({L},b_m)$. In case 3, $N({L},b_m)$ is set to zero. A point projected on $b_m$ with end-points $p_1$ and $p_2$ can be denoted as $p_1 + w(p_2-p_1)$. In the last case, for the end-point of ${L}^{'}$ locating outside $b_m$ ($w<0$ or $w>1$), we calculate its distance to the end-points of $b_m$ and assign the minimum value to $N({L},b_m)$.
${L}$ with value of a)-c) smaller than given thresholds will be denoted as a boundary matching line $\hat{L}$.}
% (purple lines in Fig.~\ref{fig:LoLs})

The set of lines of $LoL_1$ are further refined by: i) eliminating tiny noisy $\hat{L}$ matching any $b_m$, ii) merging the set of lines $\hat{L}$ matching the same $b_m$ into one single line segment, iii) extending $\hat{L_1}$ and $\hat{L_2}$ until they share a same end-point, if the matching boundary $b_p$ and $b_q$ of $\hat{L_1}$ and $\hat{L_2}$ are neighbors, and iv) connecting $\hat{L_1}$ and $\hat{L_2}$ whose matching boundary are $b_p$ and $b_q$ respectively, if the inserted $L$ can match $b_o$ whose neighbors are $b_p$ and $b_q$.
\wdx{The above operations are illustrated in Fig.~\ref{fig:LoLs} and the refined $\hat{L}$ are visualized in purple.}
The $LoL_1$ can serve as a guidance for texture stitching in sec.~\ref{sec:texture-stitching}.

%\wdx{A point projected on a line segment with end-points $p_1$ and $p_2$ can be denoted as $p_1 + w(p_2-p_1)$. For the end-points of ${L}^{'}$ locating outside $b_m$ (with $w<0$ or $w>1$), we calculate their point-to-point distance to their closest end-point of $b_m$ and assign the minimum value to $N({L},b_m)$ as shown in Fig.~\ref{fig:LoL1}(3)).} %Lines with similar gradients share a higher similarity.
%ii) The maximum point-to-point distance on the two pairs of end-points. This can measure the integral similarity of two lines, and differentiate lines with similar slopes and lengths but large spatial distances.


%This is to increase the shape similarity compared to the proxy boundary (e.g., close the loop of extracted three lines to represent a complete frame).
%Finally, those incomplete line segments \jwc{what are the incomplete line segments?} similar to specific lines belonging to the proxy boundary are extended until $LoL_2$ could maximally match $\mathcal{B}_j$.

\paragraph{$LoL_2$.}
\wdx{Finally, we cluster all the line segments in $LoL_1$ to extract structural lines with a dynamic K-means algorithm, according to the slope and the distance from the image center to the line segment.}
After that, we can obtain $LoL_2$ to represent the structural layouts of facade components and to serve as a reference for later inpainting in sec.~\ref{sec:texture-optimization}. Until now, for each selected image, we obtain LoLs for different operators. \wdx{Fig.~\ref{fig:LoLs} illustrates the LoLs from a facade image of Hitech.}

%Please refer to the supplemental for the extracted LoLs on more examples.

\ignore{
\begin{algorithm}[tbh!]
\hq{	
	\KwIn{texture image $I, \alpha, \beta, \gamma, \varphi, \omega$}
	\KwOut{$LoL_0, LoL_1, LoL_2$}
	\SetAlgoLined
	Extract initial lines \{$L$\} in texture image $I$ ~\cite{suarez2022elsed} (Section ~\ref{sec:LOLs})\\
	
	Get $LoL_0$ \{$L$\} by merging collinear lines \{$L~|~\dfrac{\overrightarrow{L_i}\cdot\overrightarrow{L_j}}{\lvert L_i \rvert\cdot\lvert L_j \rvert}<\alpha,d_1(L_i,L_j)<\beta,d_2(L_i,L_j)<\gamma$\} and filtering lines \{$L~|~\lvert \overrightarrow{L} \rvert<\varphi$\} ~\cite{jia2021leveraging}\\
	
	Calculate rigid transformation for $I$ and $LoL_0$, get transformed $I'$ and \{$L'$\} ~\cite{besl1992method} (Section ~\ref{sec:texture-stitching})\\
	
	Get $LoL_1$ \{$L'$\} by refining \{$L'$\} based on proxy boundary $B$ (Section ~\ref{sec:LOLs})
	
	\For{each boundary $B_i$}{
		\For{each boundary line $L^b \in B_i$}{
			Calculate $S_{i,b}$ \{$L'|Similarity(L',L^b)>\omega$\}\\
			\If{$S_{i,b}\neq\varnothing$}
			{Merge lines in $S_{i,b}$}
		}
		\For{each boundary line $L^b \in B_i$}
		{\If{$S_{i,b}=\varnothing$}
			{Get two endpoints $p_{b-1}$ and $p_{b+1}$ of $S_{i,b-1}$ and $S_{i,b+1}$ closest to $L^b$\\
				Insert line $L'$ ($p_{b-1}$, $p_{b+1}$) to $S_{i,b}$}}
	}
	Get $LoL_2$ by clustering $LoL_1$ using K-means (Section ~\ref{sec:LOLs})
	\caption{LoLs Extraction}
	\label{alg:LoL}
}
\end{algorithm}
}



\subsection{Line-guided Texture Stitching}
\label{sec:texture-stitching}

For each proxy polygon $\mathcal{P}_i$, %surrounded by boundary shape $\mathcal{B}_i$,
we have obtained a subset of views $\{ \mathcal{I} \}_i$ along with their LoLs in previous steps.
For simplicity, we denote the first selected image $\mathcal{I}_1$ in $\{ \mathcal{I} \}_i$ as a reference image $\mathcal{I}^{ref}$ and the others as target images $\mathcal{I}^{tar}$.
To generate an enlarged texture map, we need to find the matching relationship between two images to stitch them together.
Based on extracted LoLs, one solution is to find the correspondence between the lines (\eg using LBD descriptor~\cite{zhang2013efficient}) by considering both image and geometry features.
However, there exists plenty of repetitive patterns which make such pixel-based methods less effective. Therefore, we develop an algorithm for matching line segments by utilizing geometric information.

%Since the views are calibrated beforehand and projected onto the polygon, the influence of large variance on viewing directions in image stitching has been mitigated\jwc{I do not understand the logic between this sentence and the next sentence}.

Due to the camera and geometry inaccuracy, there exists obvious texture-to-geometry displacement which increases the difficulty in accurate image local matching and stitching. We start by globally registering $\mathcal{I}^{ref}$ towards $\mathcal{B}_i$ with a rigid transformation and several warping operators. Next, following the order of their insertion into $\{ \mathcal{I} \}_i$, all the $\mathcal{I}^{tar}$ are sequentially deformed to match $\mathcal{B}_i$ globally, then locally stitched to $\mathcal{I}^{ref}$. The $n$-th inserted image is denoted as $\mathcal{I}_{n}$.
%In the following paragraph, we introduce the details of each operator.
The stitching process is done in three steps: rigid alignment, line matching and texture warping.


%One intuitive solution is to extract texture patches from $\mathcal{R}_i$ for each part of $\mathcal{P}_i$ as previous method \cite{waechter2014let}. However, such strategy suffers from two obstacles. First, the corresponding extrinsic parameters are not perfectly accurate which cause obvious seams at the borders of texture patches. Second, important geometric priors such as boundary edges in texture maps are not explicitly extracted and preserved across adjacent patches. Therefore, we propose a plane-based image stitching mechanism to generate one complete texture map for $\mathcal{P}_i$ by aligning the line-segments detected in each image during the warping procedure.

%and yields little correspondence boundary shape among texture image and proxy polygon.

%This highly increases the accuracy of line matching.


%Texture alignment with LOL2;
\paragraph{Rigid alignment.}
To reduce the large texture-to-geometry misalignment, each image $\mathcal{I}_{n}$ is transformed toward the proxy boundary $\mathcal{B}_i$. Firstly, we extend each image with a margin of $N$ pixels and extract complete $LoL_0$ from the extended version. We compute the bounding box of $\mathcal{B}_i$ and set $N$ to $5\%$ of the length of its diagonal. This can be observed in Fig.~\ref{fig:LoLs}.
Next, we convert all the endpoints of $LoL_0$ in $\mathcal{I}_n$ into a source point cloud $\mathcal{C}_n$. We then convert the endpoints of $\mathcal{B}_i$ into a target point cloud $\mathcal{C}_i$. A rigid transformation is calculated via ICP~\cite{besl1992method} to align $\mathcal{C}_n$ toward $\mathcal{C}_i$. This rigid transformation is employed to transform and update $\mathcal{I}_n$.
%Fig.~\ref{fig:Pre-alignment} shows the alignment result on a proxy polygon of Hitech.

%Image stitching with an adaptive mesh constructed with LOL0;
%\paragraph{Line segment matching.} For each line segment $ {L}^{tar} \in \mathcal{ {L}}^{tar}$, it can be registered to line segment $L^{ref} \in \mathcal{L}^{ref}$ if satisfying: i) the angle $\theta({L}^{tar},L^{ref})$ between two supporting lines is smaller than $5^{\circ}$, ii) the maximum point-to-line distance $D_{l}({L}^{tar},L^{ref})$ from four end-points to another line is closer than 10 pixels, \wdx{and iii) the level of non-overlap $N({L}^{tar},L^{ref})$ is smaller than 100 pixels if $L^{ref} \in \mathcal{B}_j$. We denote $\mathcal{L}$ as the set of all pairs of matched line segments between $ {\mathcal{L}}^{tar}$ and $\mathcal{L}^{ref}$.}

\paragraph{Line segment matching.} We denote $LoL_1$ of $\mathcal{I}^{tar}$ as $\mathcal{ {L}}^{tar}$ and $\mathcal{I}^{ref}$ as $\mathcal{ {L}}^{ref}$. For each line segment $ {L}^{tar} \in \mathcal{ {L}}^{tar}$, it can be registered to line segment $L^{ref} \in \mathcal{L}^{ref}$ if satisfying: i) the angular distance $\theta({L}^{tar},L^{ref})$ is smaller than $5^{\circ}$, ii) the point-to-line distance $D_{l}({L}^{tar},L^{ref})$ is closer than 10 pixels, and iii) the level of non-overlap $N({L}^{tar},L^{ref})$ is smaller than 100 pixels if $L^{ref} \in \mathcal{B}_i$. We denote $\mathcal{L}$ as the set of all pairs of matched line segments between $ {\mathcal{L}}^{tar}$ and $\mathcal{L}^{ref}$.

%We employ an adaptive mesh data structure to perform the image-to-polygon-warping operator, preserving the straightness and completeness of the extracted line segments of $LoL1$.

\paragraph{Texture warping.} With the matched lines in $LoL_1$, we can warp $\mathcal{I}^{tar}$ to $\mathcal{I}^{ref}$ while preserving the matched line segments. The warping of $\mathcal{I}_n$ to $\mathcal{B}_i$ shares the same process\ignore{ with matched lines in $LoL_1$}.
Previous work~\cite{jia2021leveraging} converts the transformation into a global line-guided mesh deformation problem. They rely on deforming the vertices of a grid-mesh uniformly sampled in the target image to maintain line structures by solving a global least-square energy function.

However, the global optimal deformation method may not guarantee the strict straightness of colinear line features in facade images.
\begin{wrapfigure}{r}{0.25\linewidth}
	\centering
	\includegraphics[width=\linewidth]{images/adaptive-mesh}
	%\label{fig:adaptive-mesh}
\end{wrapfigure}
In this work, we employ an adaptive-mesh data structure to explicitly maintain the line segments after warping. First, we construct a constrained Delaunay triangulation $M^{tar} = (V^{tar},E^{tar},F^{tar})$ based on $LoL_1$, keeping all the inserted segments as constraint edges, as shown in the right wrapped figure. Unlike uniformly sampling grid-mesh data structure, every basic element in our adaptive mesh encodes a meaningful geometric primitive in the target image, \ie a corner point or a line segment.
Based on this, all the vertices $V^{tar}$ are deformed to new positions $\widetilde{V}^{tar}$ while satisfying the following two constraints:
\begin{itemize}[leftmargin=*]
	\item The matched line segment pairs in $\mathcal{L}$ are well aligned after the mesh deformation.
	\item All the line segments in $ {\mathcal{L}}^{tar}$ preserve straightness after the mesh deformation.
\end{itemize}

We search for the optimal deformation offset $\Delta{V}=\widetilde{V}^{tar}-V^{tar}$ by embedding these two constraints and a normalization term into an energy minimization formulation:
\begin{equation}
	E(\Delta{V})=\lambda_a E_a(\Delta{V}) + \lambda_l E_l(\Delta{V})   + \lambda_r E_r(\Delta{V})\text{.}
 \label{eq:deformation}
\end{equation}
%where the offset of vertices is represented by \[\Delta{V}=[\Delta{V_{1x}},\Delta{V_{1y}},\Delta{V_{2x}},\Delta{V_{2y}},\ldots]^{T}\]
$E_a(\Delta{V})$ represents the line-alignment term, which guarantees the alignment between all pairs of matched line segments in $\mathcal{L}$ after deforming vertices by $\Delta{V}$ in the form of
\begin{equation}
	E_a(\Delta{V}) = \sum_{t=1}^{|\mathcal{L}|}d(V^{tar}_{t1}+\Delta{V_{t1}}, l_t^{ref})+ d(V^{tar}_{t2}+\Delta{V_{t2}}, l_t^{ref}) \text{,}
\end{equation}
where $l_t^{ref}$ is the $t$-th matched line segment in $\mathcal{L}^{ref}$, and $(V^{tar}_{t1},V^{tar}_{t2})$ are end points of $t$-th matched line segment in $ {\mathcal{L}}^{tar}$. Moreover, the line-preserving term denoted as $E_l(\Delta{V})$ ensures the straightness of each line segment in $ {\mathcal{L}}^{tar}$ after mesh deformation by
\begin{equation}
	E_l(\Delta{V}) =\sum_{j=1}^{| {\mathcal{L}}^{tar}|} [ (V^{tar}_{j1}+\Delta{V_{j1})-(V^{tar}_{j2}+\Delta{V_{j2})} ]^T \cdot \overrightarrow{n}_j^{tar}} \text{,}
\end{equation}
where $(V^{tar}_{j1},V^{tar}_{j2})$ are end points of $j$-th line segment $l_j^{tar}$ in $ {\mathcal{L}}^{tar}$ and $\overrightarrow{n}_j^{tar}$ is the normal vector of $l_j^{tar}$.
%The normalization term denoted as $E_r$ prevents exaggerate deformation in the form of $E_r(\Delta{V}) = \sum_{t=1}^{|\mathcal{L}|} ||\Delta{V}||^2$,
%\begin{equation}
%	E_r(\Delta{V}) = \sum_{t=1}^{|\mathcal{L}|} ||\Delta{V}||^2 \text{,}
%\end{equation}
The normalization term to prevent exaggerate deformation is defined as $E_r(\Delta{V}) = \sum_{t=1}^{|\mathcal{L}|} ||\Delta{V}||^2$. $\lambda_a$, $\lambda_l$, and $\lambda_r$ in Eq.~\ref{eq:deformation} is set to 0.5, 0.5, and 0.025 in all experiments.

%The optimal offset is then solved by the conjugate gradient algorithm.
Instead of optimizing the vertex position via LSQM~\cite{jia2021leveraging}, we calculate the vertex offset by applying the conjugate gradient algorithm which is more stable and efficient.
Unlike using the calculated vertex position to update enclosing grid vertices with bilinear interpolation~\cite{jia2021leveraging}, each line segment represents a linear feature of a facade component in our case. We directly apply the optimal vertex offsets to the end-points of lines for the preservation of linear features.
There can appear topological issues of the updated mesh after that. Hence, we introduce a refinement step to address the topological issues such as line crossing and non-manifolds.
%Since $l^{tar}$ can differ a lot from $l^{ref}$, there can appear topological issues of the updated mesh after applying the offset. Hence, we introduce a refinement step to address the topological issues including: i) lines crossing, we update the relative end-points to the point of intersection; ii) lines isolation, we extend the two lines and move the breaking vertex to the point of intersection. In this way, we can better fit the optimized lines towards the target line features.
Finally, with an affine transformation constructed by the refined vertices of adaptive mesh facet $f \in F^{tar}$, each pixel $p^{tar}$ inside the $f$ is warped to the new position $\widetilde{p}^{tar}$.
With the alignment and warping operators, all the visible regions are globally warped to $\mathcal{B}_i$ and locally warped to $\mathcal{I}^{ref}$ forming an enlarged texture image for each proxy polygon $\mathcal{P}_i$.


\ignore{\begin{figure}[tp]
		\centering
		\includegraphics[width=.6\linewidth]{figs/adaptive_mesh.pdf}
		%\vspace{4mm}
		\caption{Adaptive mesh data-structure. We construct a constrained Delaunay triangulation by inserting detected line-segments and edges of boundary polygons as constraints.\wdx{need to use projected images to extract lines.}}
		\label{fig:adaptive_mesh}
\end{figure}}


\ignore{\begin{figure}[tp]
	\centering
	\includegraphics[width=.99\linewidth]{images/fig9}
	%\vspace{-3mm}
	\caption{\wdx{Texture maps with global and local misalignment before (left) and after (right) performing line-guided image stitching.}}
	\label{fig:warping}	
\end{figure}}



\subsection{Texture Optimization}
\label{sec:texture-optimization}

%The previous step enables us to generate a texture map $\mathcal{I}_i$ for each planar shape $\mathcal{P}_i$. This step aims at further improving the overall quality of $\mathcal{I}^{ref}$ relying upon a series of texture optimization operators.

%Adjust image illumination according to histogram;
%need a figure here to show the local and global luumination adjustment


\paragraph{Illumination adjustment.} Previous steps enable us to generate a texture map $\mathcal{I}_i$ for each proxy polygon $\mathcal{P}_i$. Since $\mathcal{I}_i$ is composed of patches extracted from various viewing directions, the brightness may be inconsistent across neighbouring patches. Assuming that the brightness distribution over the whole texture map should hold a specific pattern, we perform a histogram specification operation to improve the illumination consistency of $\mathcal{I}_i$ in HSV color space. To be precise, we first calculate a distribution histogram of the channel $V$ on the non-overlapping region of $\mathcal{I}^{tar}$ and overlapping region of $\mathcal{I}^{ref}$, respectively. Next, we match these two histograms and transfer the brightness of the overlapping region on $\mathcal{I}^{ref}$ to the non-overlapping region on $\mathcal{I}^{tar}$.
%by performing a look-up table transform according to the histogram matching results. \ignore{Figure~\ref{fig:illumination} shows a facade texture with illumination adjustment.}


\ignore{\begin{figure}[t!]
		\centering
		\includegraphics[width=.25\linewidth]{images/empty.png}
		\caption{A facade of Hitech before (left) and after (right) illumination adjustment.}
		\label{fig:illumination}
\end{figure}}


%\paragraph{Global Illumination Adjustment.} For a mass model with a higher level of detail, the polygon primitives in the same category might come from different views and exhibit apparent illumination differences, as shown in Fig.~\ref{fig:global-illumination}. Only considering the adjacency of polygons is not enough in these cases. We here propose a global adjustment step to harmonize the illumination across the entire model. First, we clustered all the proxy polygons based on the shape of the boundary and HSV distribution histogram. We then transfer the brightness of the clustering center to all the images in this cluster. The result of a library example with repetitive facade components is shown in Fig.~\ref{fig:global-illumination}.



%\subsection{Line-guided Texture Inpainting}
%\label{sec:texture-inpainting}

% Texture inpainting with LOL1.
% inpainting with LDM

\paragraph{Texture inpainting.} In practice, some regions in $\mathcal{P}_i$ may not be observed by any of the selected views or covered with high-quality patches, leading to holes in the generated texture map. To reduce this visual artifacts, we need to fill the missing regions (referred to as masks) to generate a complete texture map. However, the arbitrary sizes and irregular shapes of the mask pose great challenges to previous inpainting methods (\eg patch-based approaches~\cite{barnes2009patchmatch,huang2014image}). Inspired by the strong capability of diffusion model in generating semantic and geometric harmonious results, we employ a denoising diffusion probabilistic model called RePaint~\cite{lugmayr2022repaint} for free-form inpainting. We find that the quality of training data is crucial for RePaint to generate feasible results for a specific scenario, such as the architecture in our case.

%The final step of our algorithm aims at inpainting the missing regions of texture maps. The textures to be inpainted here are projected views with repetitive components and regular layouts. The missing regions have varying sizes and irregular shapes. We first employ a denoising diffusion probabilistic model called Repaint~\cite{lugmayr2022repaint} because of its strong capability in generating semantic and geometric harmonious results. However, the quality of training data is crucial for the generation of feasible results for such a specific scenario. Hence, we created a TwinTex dataset and fine-tuned the Repaint model which was trained with the ImageNet~\cite{russakovsky2015imagenet}. We denotes the fine-tuned version as TRP.

To adapt RePaint to our task, we create a TwinTex dataset and fine-tune Repaint which was originally trained on ImageNet~\cite{russakovsky2015imagenet}. %We denote the fine-tuned version as TwinTex Repaint (TRP).
Starting from $44k$ high-resolution images collected with aerial drone covering $17$ \wdx{outdoor architectural scenes}, we first project each image to all its visible $\mathcal{P}_i$ and extract the pixels inside the bounding box of visible regions. Each extracted image is then cropped to a set of images with the size of $512 \times 512$. Next, we remove the images with heavy blurring issues or containing a large portion of non-architectural contents (\eg vegetation, human, scaffolds, etc)~\cite{zhao2017pyramid}. Our final TwinTex dataset (TwinTexSet) contains $46k$ images of various scene components and building categories (school, office building, etc). Note that all the image regions with heavy blurring issue and extreme inclined angles have been removed from our data set.
\wdx{Note that there are some overlaps between the training and testing scenes. However, the TwinTex dataset contains the processed photos of 17 outdoor scenes, where we have rectified the photos, removed blurring regions and large non-architectural objects. After these processes, the training images and the test texture maps have no overlap. The missing regions in test images come from frustum-culling, visibility detection, or are not included in input photos. Therefore, the regions to be infilled never appear in the training images, thus never seen by the trained model in our tasks.}


\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{images/MMRP2.pdf}
	%\vspace{-5mm}
	\caption{Overview of our proposed texture inpainting approach, MMRP.}
	%\vspace{-5mm}
	\label{fig:inpainting-overview}
\end{figure}


\ignore{\begin{figure}%[!tbh]
	\centering
	\includegraphics[width=\linewidth]{images/inpainting.jpg}
	\caption{Inpainting results of CPGS~\cite{huang2014image} and our MMRP on a facade of Hitech with an irregular missing region.}
	%\vspace{-3mm}
	\label{fig:cpm-inpainting}
\end{figure}}


\wdx{We make use of our TwinTex dataset to fine-tune the RePaint model. The total training time is about 9 hours.  We only need to pay the time cost for training once.}
However, the above solution is still not robust enough to generate structurally consistent results for a large missing region. To alleviate this issue, we further introduce a line-guided version of RePaint called Multi-Mask RePaint model (MMRP) to preserve the geometric consistency.
%A binary mask with white pixels as \hq{known} regions and black ones as \hq{unknown} regions is usually generated according to the input texture to be filled.
As shown in Fig.~\ref{fig:inpainting-overview}, the input of MMRP contains the mask, $LoL_2$, and the texture to be completed.
We then propose a multi-mask noise initialization (MMNI) component.
\wdx{Firstly, we compute the principal directions of the lines in $LoL_2$ by using principal component analysis (PCA). Our MMNI divides the unobserved region into several parts following the second max principal direction. %with PCA~\cite{abdi2010principal}.
As mentioned by~\citet{croitoru2023diffusion}, the results will show better Frechet Inception Distance values and faster convergence with a mixture of Gaussian noises. Inspired by this observation, unlike the original RePaint that initializes the entire unobserved region with a single random Gaussian noise, we randomly initialize each divided part with a random Gaussian noise $N(\mu,\sigma)$, where $\mu$ ranges from [0, 10], $\sigma$ ranges from [1, 50]. The ranges are chosen from experimental results that deliver good performance.}


%The mask is then divided into several parts along with a dividing direction (DD, the second max principal direction).
%The mask is then divided into several parts along with the second max principal direction.
%Each divided part is initialized with a random gaussian noise.
After that, the parts initialized with multiple noises along with observed content are merged into one image, $x_{t}$, which will be harmonized together into a new inpainting.
With MMNI, our MMRP can increase the possibility of generating result that is more consistent with the observed region.


For an image with high resolution, we will resize it to $512 \times 512$. %after extracting mask and LoLs.
And for an image with large missing area, we choose to scale it according to the largest dimension while preserving the image ratio. The resized image will be fed into MMRP to receive a semantic and geometric consistent inpainting. Finally, we upsample the resultant inpainting to the original size with a bi-linear interpolation operation.
Please refer to the supplemental for more details and experimental results.


\ignore{Fig.~\ref{fig:cpm-inpainting} shows our inpainting results comparing to~\cite{huang2014image} which performs image completion using planar structure guidance (CPSG). It indicates that our MMRP result exhibits a higher level of semantic and geometric consistency.
Please refer to the supplemental for more details and experimental results.}


%For the case of a large missing region, the TRP is not robust enough for the generation of structural coherent results. Hence, we proposed a variant on RePaint to improve this issue.
%%We first divide the mask denoting the missing region into several parts, according to the major directions of $LoL_2$ extracted with PCA~\cite{abdi2010principal}.
%The mask is usually a binary image with white pixels as unknow pixels and black ones as known regions. We first divide the mask into several parts based on $LoL_2$. These masks along with the input texture to be completed are then fed into a proposed Multi-Mask RePaint model (MMRP) as shown in Fig.~\ref{fig:inpainting-overview}.
%In time step $t$, unlike the original method that initializes the entire unobserved region with a noise distribution, our MMRP initialize each part with different noise distributions. Then, all the parts will then be merged into one image and harmonized together with the observed content into $x_{t-1}$ same as Repaint. By dividing the missing region into parts, we can slightly increase the possibility of generating results which is more compatible with the observed region. Please refer to the supplemental for the details on MMRP structure.
%Experimental results of completed textures compared to PatchMatch are shown in Fig.~\ref{fig:cpm-inpainting}. Our result exhibits a higher level of semantic and geometric consistency.

%These separately initialized $x_t$ can be observed in Fig.~\ref{fig:MMRP}



%Inspired by linear geometric features based image completion method proposed in~\cite{huang2014image}, we employ a similar approach to inpaint the missing parts of each plane. Unlike their method that detects three main direction planes from three vanishing points under Manhattan-World assumption, our texture map exhibits only one planar shape. Thus, we instead detect two sets of parallel line-segments and utilize these regularities to guide the image painting using the propagation mechanism in Patch  Match~\cite{barnes2009patchmatch}.


%\paragraph{TwinTex Dataset.} This LDM is trained with our proposed architectural images dataset containing various scene components (facade, roof, road, green belt, etc) and building categories (school, office building, factory, etc).





==> src/backup/06-results.tex <==
\section{Results}
\label{sec:results}

To validate the proposed algorithm, we conduct a series of experiments on real-world scenes with varying building styles and functions.
We first demonstrate the robustness of our approach and the effectiveness of each main ingredient through a stress test.
Then, we evaluate our approach by comparing it against state-of-the-art texture mapping methods.
%Then, we demonstrate the effectiveness of our main technical ingredients through ablation studies.
%Results on an example with proxy models at different levels of detail textured by our method and manual work are also provided in the supplemental materials to demonstrate the robustness of our framework.
Ablation studies are performed as well to show the effectiveness of our main technical ingredients (please refer to the supplemental material for the details).
Texturing results by our method and manual work on proxy models at different levels of detail are also provided in the supplemental material to demonstrate the high quality of our generated texture maps. %the robustness of our framework.
Our algorithm is implemented in C++ and also well-organized as a customized plug-in for Houdini. All the presented experimental results are obtained on a desktop computer equipped with an Intel i9-10900k processor with 3.0 GHz and 128 GB RAM. Note that the time cost for fine-tuning the RePaint model are not included in the statistics.


%\noindent
\textbf{Dataset.}
For the performance evaluation and comparisons, we carry out experiments on \wdx{$17$ real-world scenes, including $15$ outdoor buildings, two indoor rooms and a man-made object}. \wdx{These scenes come from public sources (\ie Library~\cite{DronePath21}, Hitech~\cite{DroneScan20}, Polytech and ArtSci~\cite{UrbanScene3D}), a handheld device (\ie Machine Room, Lab, Cabinet), or are captured by a single-camera drone (\ie Highrise, School, Center, CSSE, Sunshine Plaza, Hall, Center, Factory, Hisense, Bank).}
Please refer to the supplemental material for detailed statistics on the photo collections and models.
Then we use the commercial software \wdx{RealityCapture\footnote{https://www.capturingreality.com/} (RC)} to reconstruct the 3D high-precision models from the captured images.
All the abstracted versions are either the coarse 2.5D models for path planning~\cite{DroneScan20}, or created by in-field modelers.
%\wdx{or generated with structure-aware surface reconstruction method~\cite{bauchet2020kinetic}}.vice
All of the dense reconstructions and proxy models are utilized to demonstrate the performance of our algorithm. %throughout the experiments.
%\wdx{Due to the limit on pages, for the large-scale scenes, we only show the overall views of the resultant proxy textured with our methodology. For the indoor scenes and objects, we visualized the overall views generated with RC, LTBC, and ours.}



\begin{figure}[!tbh]
	\centering
	\includegraphics[width=.95\linewidth]{images/stress-test2}
	%\vspace{-3mm}
	\caption{\wdx{Stress test of our methodology on Hall example via randomly removing a certain percentage of photos from original input. In each row we visualize: the camera distribution of the remaining input, the textured proxy based in remaining input after view selection, image stitching with blending, and inpainting. $\# I$ denotes the number of photos. The value in the bracket denotes the percentage of the remaining photos related to original input.}}
	\label{fig:stress-test}
\end{figure}

\subsection{Stress Test}

%We first evaluate the robustness of our approach by varying the number of views in the given photo set. This stress test is performed via randomly removing partial photos from the original photo set and feeding the rest views into our TwinTex. The textured proxies of two scenes generated with three different sets of remaining views are shown in Fig.~\ref{fig:stress-test}. We also show the intermediate texture maps after each step, \eg view selection, image stitching along with blending and texture inpainting.

%The first scene is the Factory example with 589 collected photos. We randomly removed $50\%$, $75\%$ and $95\%$ images and made use of the remaining views to texture this proxy model.

\wdx{We first evaluate the robustness of our approach on a complicated Hall example with 519 input views. This stress test is performed via randomly removing partial photos from the original photo set and feeding the rest views into our TwinTex. The textured proxies of Hall example generated with three different sets of remaining views are shown in Fig.~\ref{fig:stress-test}.} We also show the intermediate texture maps after each step, \eg view selection, image stitching along with blending and texture inpainting.

We randomly removed $50\%$, $75\%$ and $85\%$ photos from the original set and made use of the remaining views to texture this proxy model.
The textured proxies after view selection are generated by simply overlapping the projection of selected images following the reverse order of selection. As the number of photos in the remaining input decreased, our selection algorithm can still select high-quality photos from the input to maximally cover the proxy, as illustrated in the second column of Fig.~\ref{fig:stress-test}. From the third column, we can see the texture maps after performing our stitching step and illumination adjustment exhibit higher geometric and photometric consistency. However, there appears larger missing regions as the number of remaining views decrease.
\wdx{We only use $77$ images to texture Hall example with $225$ facades (each plane has about $6$ photos to select from).}
All the missing regions are visualized with black pixels, as marked by the red boxes in the figure. The final texture maps visualized in the last column of Fig.~\ref{fig:stress-test} demonstrate the ability of our inpainting framework for creating geometrically and semantically consistent contents under very limited resource.


% add description and analysis when results are ready



\begin{figure*}[tbh!]
	\centering
	%\includegraphics[width=\linewidth]{images/compare1-five.png}
	\includegraphics[width=\linewidth]{images/compare1-5}
	%\vspace{-2mm}
	\caption{Visual comparison against RC, LTBC and ours on \wdx{two} examples. The detailed comparisons are shown in the zoomed-in insets. Due to the page limit, we only show the overall views of our textured proxy models, which are shown on the left \wdx{to the zoomed-in insets}.}
	\label{fig:comparison}
\end{figure*}

\subsection{Comparison with Texturing Methods}

%1. dense model
%2. LTBC
%3. PBO
%4. Ours


In this subsection, we evaluate the quality of our generated texture maps by comparing them against RC and two competitive texturing generation frameworks, let there be color (LTBC)~\cite{waechter2014let} and patch based optimization (PBO)~\cite{bi2017patch}.
%\jwc{The textures on dense reconstructions returned by the commercial software RC are also compared.}
%\jw{The textures on dense reconstructions returned by the commercial software RC are also exhibited as a visual reference to depict the real scenes.}
%\wdx{The texture returned by RC is also exhibited as a visual reference to measure the perceptive distance from texturing results of the two methods to real scenes.}
We adopt the evaluation scheme proposed by~\citet{Waechter2017} to compare the rendered image with the corresponding real image following a specific view from the input cameras.
\wdx{We select the ground truth photos for evaluation from the input excluding the photos for texturing. }
Two visual similarity metrics, namely the structural similarity index measure (SSIM) and learned perceptual image patch similarity (LPIPS)~\cite{kastryulin2022piq}, are adopted for quantitative evaluation.
%We first render the entire textured model following a specific view from the input cameras, then compare the similarity between the rendered image and the corresponding input photo.



\textbf{Comparison with LTBC.}
We first compare our method with RC and LTBC on \wdx{two} examples.
Note that LTBC selects the most suitable view for each facet by solving a Markov Random Field formulation and adjusting the pixel values along the boundary edges of adjacent patches to alleviate the seams. This strategy fails to texture large facets when there is no camera view observing the whole region of the facet. Thus, we subdivide the simplified coarse model and perform LTBC to generate texture maps for the corresponding subdivided mesh for a reasonable comparison.
%In the dense mesh of RC, a large-scale plane is usually represented by too many small triangular facets, resulting in inconsistent and cluttered textures between adjacent facets due to the camera misalignment and 3D reconstruction inaccuracies, as illustrated in Fig.~\ref{fig:cmp_manual}.
%As a projection-based approach,~\cite{waechter2014let} selects an optimal view to texture each facet by solving a Markov Random Field formulation to alleviate the seams between adjacent patches.



\ignore{\begin{table}[!tbh]%
	\caption{Quantitative comparison on the texturing results in Fig.~\ref{fig:comparison}.}
	%\vspace{-3mm}	
	\label{tab:quality-results}
	\begin{center}
		%		\small
		\begin{tabular}{c c c c c}
			\midrule[1pt]
			\multirow{1}{*}{Scene} & \multirow{1}{*}{Method}  & $ SSIM\uparrow$ & $LPIPS \downarrow$   & Time (min)\\
			\midrule
			%\multirow{3}{*}{Hitech}   & RC      &     0.5738 &  0.4938     & 141.50 \\
			%\multicolumn{1}{c}{}        & LTBC     & 0.5989    & 0.4465    &  1.93   \\
			%\multicolumn{1}{c}{}        &  Ours                          & \textbf{0.6251}     &\textbf{0.4424}     &   99.98    \\ \hline
			\multirow{3}{*}{Center}   & RC      &    0.3500     &  0.8309    & 287.00    \\
			\multicolumn{1}{c}{}        & LTBC  &    0.3537  &   0.8360    & 4.40   \\
			\multicolumn{1}{c}{}        &  Ours     & \textbf{0.3581}       &   \textbf{0.8307}  &  167.44    \\ \hline
			\multirow{3}{*}{Artsci}   & RC     &   0.3458    & 0.8833   &   320.89   \\
			\multicolumn{1}{c}{}        & LTBC      &  0.3313   &      \textbf{0.8734}    &   5.98  \\
			\multicolumn{1}{c}{}        &  Ours                        & \textbf{0.3482}   &      0.8772    &     256.11  \\
			\midrule[1pt]
		\end{tabular}
	\end{center}
\end{table}%
}

\begin{figure*}[tbh!]
	\centering
	\includegraphics[width=.78\linewidth]{images/compare2-2}\\
	%\hspace{0.1mm}
	\includegraphics[width=.78\linewidth]{images/compare3-2}
	\caption{\wdx{Visual comparison against RC, LTBC, PBO and ours on \wdx{four} examples. The detailed comparisons are shown in the zoomed-in insets.}}
	\label{fig:comparison2}
\end{figure*}



\ignore{
\begin{table*}[!tbh]%
	\caption{Quantitative comparison on the performance of texturing results. Numbers in the bracket denote the quality value of the four zoomed-in views in Fig.~\ref{fig:comparison2} from top to bottom. }
	%\vspace{-3mm}	
	\label{tab:quality-results2}
	\begin{center}
		%		\small
		\begin{tabular}{c c c c c}
			\midrule[1pt]
			{Scene} & {Method}  & $ SSIM\uparrow$ & $LPIPS \downarrow$    & Time (min)\\
			\midrule
			%\multirow{4}{*}{Highrise}   & RC      & \{0.2762, 0.1607, 0.3408, 0.2945\} & \{0.5716, 0.6480, 0.6320, 0.6206\} &      123.00          \\
			 %& LTBC   & \{0.2854, 0.1666, 0.3455, 0.3418\}   &  \{\textbf{0.4889}, 0.6363, 0.6502, 0.5217\}       & 9.46   \\			
			 %& PBO   & \{\textbf{0.3115}, \textbf{0.2041}, 0.3918, \textbf{0.3679}\}   & \{0.5863, 0.6841, 0.6614, 0.6206\}       &   758.26      \\
			%&  Ours  &  \{0.2589, 0.1874, \textbf{0.4307}, 0.3091\}   &  \{0.5771, \textbf{0.6359}, \textbf{0.6319}, \textbf{0.2653}\}      & \ignore{27.71} 34.72          \\ \hline
			%\multirow{4}{*}{Hisense}   & RC      & \{0.0854, 0.1325, 0.0840, 0.3138\} & \{0.3379, 0.3192, 0.4550, 0.6634\} &      792.32         \\
			%& LTBC   & \{0.2908, 0.1527, 0.0812, 0.3357\}   &  \{0.3868, 0.4333, 0.4811, 0.7139\}       & 12.04   \\			
			%& PBO   & \{\textbf{0.2988}, 0.1663, \textbf{0.1165}, 0.5236\}   & \{0.4309, 0.3672, 0.4324, 0.4466\}       &   1054.63      \\
			%&  Ours  &  \{0.2932, \textbf{0.2339}, 0.0781, \textbf{0.5327}\}   &  \{\textbf{0.1203}, \textbf{0.1032}, \textbf{0.3026}, \textbf{0.2393}\}      &\ignore{431.77} \ignore{27.71} 438.82           \\ \hline					
			%\multirow{4}{*}{School}   & RC      &  \{0.1777, 0.2517, 0.3847, 0.5782\}   &  \{ 0.5837, 0.4434, 0.5512, 0.5941\}      & 375.11       \\
			%& LTBC   &  \{0.2173, 0.1857, 0.4011, 0.6426\}   &  \{0.5367, 0.5240, 0.6590, 0.5252\}       &4.80         \\			
			%& PBO   &  \{\textbf{0.4055}, 0.4816, 0.3972, \textbf{0.7445}\}   &  \{0.7204, 0.5273, 0.5758, 0.3940\}      & 893.60         \\
			%&  Ours  &  \{0.2123, \textbf{0.5947}, \textbf{0.4194}, 0.6952\}   &  \{\textbf{0.5160}, \textbf{0.2518}, \textbf{0.5150}, \textbf{0.2888}\}  & \ignore{277.22} 284.20                 \\ \hline  										
			%\multirow{4}{*}{Library}   & RC      &  \{0.2763, 0.2758, 0.3223 \ignore{, 0.5297}\}   &  \{0.5247, 0.5981, 0.6814\ignore{, 0.6496}\}       & 383.59       \\
			%& LTBC   &  \{0.2931, 0.2869, 0.3442 \ignore{, 0.4553}\}   &  \{0.5377, 0.6811, 0.6770 \ignore{, 0.4806}\}       &4.84         \\
			%\multicolumn{1}{c}{}        & PBO   &  \{\textbf{0.6261}, 0.4508, 0.3828 \ignore{,\textbf{0.7402}}\}   &  \{0.6250, 0.6996, 0.6907 \ignore{, 0.8346}\}      & 810.73        \\
			%&  Ours     &  \{0.4625, \textbf{0.3808}, \textbf{0.3635} \ignore{,0.4641}\}   &  \{\textbf{0.2806}, \textbf{0.5180}, \textbf{0.6595} \ignore{,\textbf{0.4670}}\}      &\ignore{193.38} 200.44             \\  \hline		
			%\multirow{4}{*}{Bank}   & RC      & \{\ignore{0.6085,}0.2484, 0.6184, 0.2610}\} & \{ \ignore{0.2804,}0.4257, 0.2309, 0.5348\} &      198.26         \\
			%& LTBC   & \{\ignore{0.6700, }0.2006, 0.5231, \textbf{0.3302}\} & \{\ignore{0.1912, }0.5071, 0.3740, 0.5324\}       & 6.41   \\			
			%& PBO   & \{\ignore{0.6463, }0.2461, \textbf{0.6952}, 0.2659\}   & \{\ignore{0.2157, }0.4311, 0.3050, 0.5740\}       &   672.10      \\
			%&  Ours  &  \{\ignore{\textbf{0.9650}, }\textbf{0.2598}, 0.6246, 0.2752\}   &  \{\ignore{\textbf{0.0241}, }\textbf{0.2714}, \textbf{0.1816}, \textbf{, 0.5229}}\}      &  174.51          \\ %\hline
			%\multirow{4}{*}{Apartment}   & RC      & \{0.2602, 0.5340, 0.3361, 0.4225\} & \{0.3526, 0.3618, 0.4103, 0.5158\} &      205.76          \\
			%& LTBC   & \{0.2305, 0.4461, 0.3049, 0.4211\}   &  \{0.3813, 0.4659, 0.4808, 0.6129\}       & 3.00   \\			
			%& PBO   & \{\textbf{0.4395}, 0.5333, \textbf{0.4471}, \textbf{0.6340}\}   & \{0.3332, 0.3884, 0.6198, 0.4811\}       &  806.00      \\
			%&  Ours  &  \{0.3465, \textbf{0.6718}, 0.4384, 0.5780\}   &  \{\textbf{0.1072}, \textbf{0.1516}, \textbf{0.2136}, \textbf{0.3436}\}      &  185.42          \\
			\midrule[1pt]
		\end{tabular}
	\end{center}
\end{table*}%
}



\begin{figure*}[!tbh]
	\centering
	\includegraphics[width=\linewidth]{images/compare4}
	%\vspace{-6mm}
	\caption{\wdx{Visual comparison of two challenging cases against RC, LTBC and ours. The detailed comparisons are shown as zoomed-in insets.}}
	\label{fig:challenging-cases}
\end{figure*}

Fig.~\ref{fig:comparison} shows the qualitative results on \wdx{two} abstracted models with sharp textures and structural features.
First, we can observe that LTBC and RC are not able to produce satisfactory results for large-scale planar structures which are invisible for the input photos or with only low-quality pixels. In these cases, their texture maps show blurring and ghosting artifacts. By contrast, our method can fill large unobserved regions with geometrically and semantically consistent pixels.

Second, without the constraints on perspective consistency in view selection, LTBC failed in selecting photos with both consistent and front-parallel viewing directions, creating "stretching" alike artifact and perspective inconsistency in the generated textures. The "stretching" problem can be observed in the inset of the ArtSci building in Fig.~\ref{fig:comparison} (\wdx{first row}, second column), which was caused by merging photos with large viewing angle variance. The perspective inconsistency can be observed in the insets of the Center example in Fig.~\ref{fig:comparison} (\wdx{first and third rows}, second column). Unlike LTBC, our view selection strategy can pick out a very small set of perspective consistent and front-parallel photos as possible. Moreover, we introduced a smooth term considering the pixel-wise distance of each image pair. This helps select a set of photos with a higher level of photometric and content consistency, especially for filtering out occluders or dynamic instances (e.g., cars). The significant improvement can be observed in the Center example in Fig.~\ref{fig:comparison} (\wdx{second row}) and ArtSci example in Fig.~\ref{fig:comparison} (\wdx{third row}).



\begin{table}[!tbh]%
	\caption{Quantitative comparison on the texturing results in Fig.~\ref{fig:comparison}.}
	%\vspace{-3mm}	
	\label{tab:quality-results}
	\begin{center}
		\begin{tabular}{c c c c c}
			\midrule[1pt]
			\multirow{1}{*}{Scene} & \multirow{1}{*}{Method}  & $ SSIM\uparrow$ & $LPIPS \downarrow$   & Time (min)\\
			\midrule
			\multirow{3}{*}{Center}   & RC      &    0.350     &  0.831    & 287.0    \\
			\multicolumn{1}{c}{}        & LTBC  &    0.354  &   0.836    & 4.4   \\
			\multicolumn{1}{c}{}        &  Ours     & \textbf{0.358}       &   \textbf{0.831}  &  167.4   \\ \hline
			\multirow{3}{*}{Artsci}   & RC     &   0.346    & 0.883   &   320.9   \\
			\multicolumn{1}{c}{}        & LTBC      &  0.331   &      \textbf{0.873}    &   6.0  \\
			\multicolumn{1}{c}{}        &  Ours                        & \textbf{0.348}   &      0.877    &     256.1  \\
			\midrule[1pt]
		\end{tabular}
	\end{center}
\end{table}




\begin{table}[!tbh]%
	\caption{Quantitative comparison on the performance of texturing results \wdx{on the third and fourth examples in Fig.~\ref{fig:comparison2}}. Numbers in the bracket denote the quality value of the \wdx{three} zoomed-in views \wdx{of each example} from top to bottom. \wdx{All the times are in minutes.}}
	%\vspace{-3mm}	
	\label{tab:quality-results2}
	\begin{center}
		%		\small
		\begin{tabular}{c c c c c}
			\midrule[1pt]
			Scene & Method  & $ SSIM\uparrow$ & $LPIPS \downarrow$    & Time\\
			\midrule
			%\multirow{4}{*}{\rotatebox{90}{\small{Hisense}}}   & \small{RC}      & \small{\{\ignore{0.09,} 0.13, 0.08, 0.31\}} & \small{\{\ignore{0.33,} 0.32, 0.46, 0.66\}} &      \small{792}         \\
			%& \small{LTBC}   & \small{\{\ignore{0.29,} 0.15, 0.08, 0.34\}}   &  \small{\{\ignore{0.39,} 0.43, 0.48, 0.71\}}       & \small{12}   \\			
			%& \small{PBO}   & \small{\{\ignore{\textbf{0.30},} 0.17, \textbf{0.12}, 0.52\}}   & \small{\{\ignore{0.43,} 0.37, 0.43, 0.45\}}       &   \small{1055}      \\
			%&  \small{Ours}  &  \small{\{\ignore{0.29,} \textbf{0.23}, 0.08, \textbf{0.53}\}}   &  \small{\{\ignore{\textbf{0.12}, }\textbf{0.10}, \textbf{0.30}, \textbf{0.24}\}}      &\ignore{431.77} \ignore{27.71} \small{439}           \\ \hline					
			%\multirow{4}{*}{\rotatebox{90}{\small{School}}}   & \small{RC}      &  \small{\{\ignore{0.18, }0.25, 0.38, 0.58\}}   &  \small{\{ \ignore{0.58,} 0.44, 0.55, 0.59\}}      & \small{375}       \\
			%& \small{LTBC}   &  \small{\{\ignore{0.22,} 0.19, 0.40, 0.64\}}   &  \small{\{\ignore{0.54,} 0.52, 0.66, 0.53\}}       &\small{5}         \\			
			%& \small{PBO}   &  \small{\{\ignore{\textbf{0.41},} 0.48, 0.40, \textbf{0.74}\}}   &  \small{\{\ignore{0.72,} 0.53, 0.58, 0.39\}}      & \small{894}         \\
			%&  \small{Ours}  &  \small{\{\ignore{0.21,} \textbf{0.59}, \textbf{0.42}, 0.70\}}   &  \small{\{\ignore{\textbf{0.52},} \textbf{0.25}, \textbf{0.52}, \textbf{0.29}\}}  & \ignore{277.22} \small{284}                 \\ \hline		  									
			\multirow{4}{*}{\small{Library}}   & \small{RC}      &  \small{\{ 0.28, 0.28, 0.32\ignore{,0.53} \}}   &  \small{\{ 0.53, 0.60, 0.68\ignore{,0.65} \}}       & \small{383.6}       \\
			& \small{LTBC}   &  \small{\{ 0.29, 0.29, 0.34\ignore{,0.46} \}}   &  \small{\{ 0.54, 0.68, 0.68\ignore{,0.48} \} }      & \small{4.8}         \\
			\multicolumn{1}{c}{}        & \small{PBO}   &  \small{\{ \textbf{0.63}, \textbf{0.45}, 0.38\ignore{,\textbf{0.74}} \}}  &  \small{\{ 0.63, 0.67, 0.69\ignore{,0.84} \}}     & \small{810.7}        \\
			&  \small{Ours}     &  \small{\{ 0.46, 0.38, \textbf{0.36}\ignore{,0.46} \}}   &  \small{\{ \textbf{0.28}, \textbf{0.52}, \textbf{0.66}\ignore{,\textbf{0.47}} \}}     & \small{200.4}             \\
			\hline		
			\multirow{4}{*}{\small{Bank}}   & \small{RC}      & \small{\{ \ignore{0.61,}0.25, 0.62, 0.26 \}} & \small{\{ \ignore{0.28,}0.43, 0.23, 0.54 \}} &      \small{198.3}         \\
			& \small{LTBC}   & \small{\{ \ignore{0.67,}0.20, 0.52, \textbf{0.33} \}} & \small{\{ \ignore{0.19,}0.51, 0.37, 0.53 \}}       & \small{6.4}   \\			
			& \small{PBO}   & \small{\{ \ignore{0.65,}0.25, \textbf{0.70}, 0.27 \}}   & \small{\{ \ignore{0.22,}0.43, 0.31, 0.57 \}}       &   \small{672.1}      \\
			&  \small{Ours}  &  \small{\{ \ignore{\textbf{0.97},}\textbf{0.26}, 0.63, 0.28 \}}   &  \small{\{ \ignore{\textbf{0.02},}\textbf{0.27}, \textbf{0.18}, \textbf{0.52} \}}    &  \small{174.5}          \\
			\midrule[1pt]
		\end{tabular}
	\end{center}
\end{table}%


%I assume that the photometric similarity term is enough to filter out occluders (as seems to be the
%case for the trees in the second result of Fig.11, or the cars in the third result

Furthermore, due to the lack of explicit constraints on the linear features of buildings, the texture generated by LTBC destroys geometric structures, making them suffer from serious seams and distortion effects.
Our image stitching mechanism succeeds in preserving the straightness and completeness of the line segments by constructing an adaptive mesh taking the original geometric primitives as constraints.
Next, large and duplicate texture patterns are also well maintained in our results. This is mainly because we select a suitable small subset of camera views for each planar shape instead of each facet. This strategy guarantees that each selected view is used to texture the current plane as much as possible.

%The quantitative comparison results are given in Table~\ref{tab:quality-results}. Since SSIM is by nature less sensitive to blurring issues and possibly give higher scores to images with such artifacts~\cite{zhang2018unreasonable}, the texture with heavy blurring problem could have higher scores. This phenomenon can be observed in some views per each example. Meanwhile, LPIPS are designed to match human perception and yield better scores for images with higher level of coherence. Please refer to the supplemental material for the overall views of the above three examples.




The quantitative comparison results are given in Table~\ref{tab:quality-results}. In most of the cases, the rendered views of our textured model can deliver better SSIM and LPIPS scores. Please refer to the supplemental material for the overall views of the above \wdx{two} examples.




\textbf{Comparison with PBO.}
Next, we perform comparison with PBO\footnote{https://github.com/yanqingan/EAGLE-TextureMapping} and report SSIM and LPIPS as well on \wdx{four} more architectural scenes.
We first tried to globally compare the similarity of rendering views on the entire building with real photos. However, PBO requires an extremely large amount of time/storage given just several high-resolution images as input. Remember that our target is to retain the quality of the inputs, one way to address the issues is to decrease the number of input photos. This can produce other problems such as missing contents since no pixels can cover some of the regions. It is crucial to provide key views with high quality to the PBO in this scenario.
Hence, we locally perform the comparison to PBO using \wdx{three} planes per example. To this end, we fed PBO with the set of views selected by our algorithm for the planar polygons involved in the comparison.
Considering the nature of patch-based optimization, for a fair qualitative comparison, we use the subdivided mesh prepared for LTBC as the input to PBO as well.
Fig.~\ref{fig:comparison2} shows the texturing results of RC, LTBC, PBO and ours. The comparison shows that given the same set of selected views, PBO can generate a texture with good quality in most cases which also proves the effectiveness of our view selection algorithm. However, the results of PBO have obvious blurring issue and line distortion artifact compared to the real photos. There are also some optimization failures of PBO which cause missing textures for the subdivided triangles. In comparison, our stitching and optimization frameworks can preserve clear line features and retain the original structure while we are able to inpaint missing regions.



Quantitative results are listed in Table.~\ref{tab:quality-results2}.
\wdx{Since SSIM is by nature less sensitive to blurring issues and possibly gives higher scores to images with such artifacts~\cite{zhang2018unreasonable}, the texture with the regional blurring problem could have higher scores. This phenomenon can be observed in some views per each example. Meanwhile, LPIPS is designed to match human perception and yield better scores for images with higher level of coherence.}
Note that the recorded time cost for PBO does not include view selection or is not for texturing the entire proxy although it is relatively long.



%Table~\ref{tab:cmp-time} reports the scene information and performance statistics of different methods. Compared to other methods, our approach is able to texture extremely coarse models (see the number of facets) while achieving minimal storage overhead.

%\wdx{We considered learning methods such as Nerf~\cite{mueller2022instant} as well. Reminds that we aim at very high-resolution input and output images which require extremely large memory. Employing a small set of input images however is not enough for methods in this category to generate satisfying results, which makes them less applicable in our scenario. We suggest readers check our supplemental for the details on input images.}



%\subsection{Challenges and Limitations}
\subsection{Analysis of Generalization Ability}

In this subsection, we discuss the results of our method applied to more diverse scenes. First, we conduct experiments on several challenging urban scenes that contain curve surfaces, facades with non-linear features, and facades with a lot of reflection, as shown in Fig.~\ref{fig:challenging-cases}. Then we present the texturing results on two indoor scenes and one man-made object in Fig.~\ref{fig:more-cases}, which are different scenarios from buildings. Note there exists only one fire extinguisher in the Lab scene. Although it has been moved during the photos collection process, our method still perfectly keeps its location where it has been placed in most photos.


\begin{figure}[!tbh]
	\centering
	\includegraphics[width=\linewidth]{images/extra}
	\caption{\wdx{Visual comparison against RC, LTBC and ours on two indoor scenes and a cabinet.}}
	\label{fig:more-cases}
\end{figure}



\begin{figure}[!tbh]
	\centering
	\includegraphics[width=\linewidth]{images/fig18-2}
	\caption{Failure examples: inter-planar misalignment among two adjacent facades (left), and inpainting results of a reflective facade \jw{with large glass panels} (right).}
	\label{fig:limitations}
\end{figure}



To better understand the superiority of our TwinTex, we conduct comparisons with previous methods as well. From the figures we can see that our approach can still generate high-fidelity textures for the challenging buildings, and can be naturally extended to texture coarse piece-wise planar models in other scenarios.
The visual comparisons further suggest that the textures generated by our approach have several significant advantages over previous methods: i) closer to real photos with perspective consistency and harmonic illumination, ii) contain rarely border misalignment, distortion, blurring and seaming artifacts resulting from inaccurate camera parameters, iii) contain rarely ghosting effects resulting from dynamic instances, iv) preserve geometric details better, and v) fill the missing regions with geometrically and semantically consistent contents.





%
%The texturing of simplified model has wide applications and great importance but existing methods fall short. Although our inputs comes from UAV scenarios, TwinTex can be easily extended to texture any coarse piece-wise planar models in other scenarios.
%Our TwinTex can take images that collected with any camera devices equipped with IMU following arbitrary cameras distributions (oblique photography, etc, as shown in Fig.3 Supplemental) as input, to generate image-level texture of any piece-wise planar proxy model with arbitrary topology.
%To demonstrate our application, in this revision, we have provided new experimental results and comparisons on two indoor scenes and one man-made cabinet, which demonstrate our generality and superiority as well.


%\wdx{We further performed experiments on \wdx{three} exciting and challenging cases to validate the generality of our methodology: 1) Model with curvy surfaces. 2) Facades with non-linear features. 3) Buildings full of facades with reflection. These results are exhibited in Fig.~\ref{fig:challenging-cases}. 4) Indoor scenes and a man-made object. These results are exhibited in Fig.~\ref{fig:more-cases}. Note there exists only one fire extinguisher in the Lab scene, but it has been moved during the photos collection process. Our method perfectly keep its location where it been placed in the majority of time. }

%Overall, from the visual results, we can see that the textures generated by our approach have several significant advantages: i) closer to real scenes with harmonic illumination and perspective consistency, \wdx{ii) contain rarely border misalignment, distortion, blurring and seaming artifacts resulting from inaccurate camera parameters, iii) contain rarely ghosting effects resulting from dynamic instances}, iv) preserving geometric details, and v) filling the missing region with geometrically and semantically consistent contents.

	
%\wdx{\textbf{Limitations.} However, as shown in Fig.~\ref{fig:limitations}, there still exists couple of cases that our methodology cannot handle well: 1) Global alignment of linear features among adjacent planes. 2) \ignore{Global illumination consistency among similar facades. 3) }Inpainting of reflected facades which lacks of coherent structures and clear content which makes it even hard for human to infer the missing region.}

	
% These methods can generate texture maps with lots of
% details. However, these methods cannot perfectly address the misalignments of
% images resulting in blurring and ghosting artifacts. Lempitsky and Ivanov [15]
% diminish visible seams by performing a global color adjustment following with
% Poisson editing [21]. However, blurring and ghosting artifacts around seams may
% still occur due to noisy input data. Other approaches are proposed to gener-
% ate seamless texture maps using geometry information. For example, Barnes et
% al. [3] provide an interactive method to manually correct misaligned errors be-
% tween the geometry model and images, which is not suitable for E-Commerce
% applications. Bi et al. [5] propose a patch-based optimization that incorporates
% geometry information. Their method estimates the bidirectional similarity of dif-
% ferent images, which suffers from high computational cost.


% RC would produce distorted and misaligned artifacts due to the camera misalignment and 3D reconstruction inaccuracies.

% However, this method is not able to produce satisfactory results in this case, since they assign inconsistent textures to some of the adjacent faces because of significant inaccuracies.

% Furthermore, they all fail to align large-scale geometric features, resulting in obvious seams in the generated texture maps

% Figure 5 shows the resulting image optimized with our approach in comparison to a naive L1 loss

% Waechter et al. [2014] select one view per
% face by solving an optimization system to hide the seams between
% adjacent faces. However, their method is not able to produce satisfactory results in this case, since they assign inconsistent textures to
% some of the adjacent faces because of significant inaccuracies. Note
% the tearing artifacts at the top inset and the distorted bear face at
% the bottom inset. Moreover, the local warping in Zhou and Koltun’s
% approach [2014] is not able to correct significant misalignment in
% this case, caused by inaccurate geometry (see Fig. 10). Therefore,
% their results suffer from ghosting and blurring artifacts. Our method
% synthesizes aligned target images and is able to produce high-quality
% texture maps with minimal artifacts. 

==> src/backup/07-future.tex <==
%\section{Conclusion}
\section{Conclusion and Future Work}

In this work, we proposed a plane-based and geometry-aware texture generation method. Our target is to produce high-resolution texture maps for piece-wise planar architectural proxy models which were abstracted from dense 3D reconstructions. Our main technical contributions consist in:
i) A greedy algorithm to select a set of views that are most suitable for texturing each planar shape; Both perspective and photometric qualities are considered in this algorithm.
ii) An image stitching methodology that can stitch the selected views to an enlarged texture map, preserving the local and global linear geometric primitives based on an adaptive-mesh data structure;
iii) An improved diffusion probabilistic model that fine-tuned with our created TwinTexSet to inpaint unobserved texture region with semantically and geometrically coherent pixels;
iv) A customized texturing tool plugged in a widely used graphical engine. Experimental results show that our algorithm outperforms state-of-the-art facet-based texturing methods in the generation of realistic and high-resolution texture maps in a reasonable time.


%Our algorithm and tool has several limitations.
%First, although we significantly refined the extracted line segments, the line-guided scheme still relies on the quality of the line extraction algorithm. One solution is to consider camera information as well or make use of reconstructed 3D lines.
%Second, our plane-based texture generation method processes each planar shape independently, which does not take their mutual relationship into consideration in a more global manner.
%Third, the processing time can be further improved with parallel processing. We will incorporate these issues in our future pipeline.

\textbf{Limitations and future work.}
\wdx{Our system still has several limitations.}
First, although we significantly refined the extracted line segments, the line-guided scheme still relies on the quality of the line extraction algorithm. One possible solution is to consider camera information as well or make use of reconstructed 3D lines.
Second, our plane-based texture generation method processes each planar shape independently, which does not take their mutual relationship into consideration\ignore{ in a more global manner}. Fig.~\ref{fig:limitations} (left) shows such an example where global alignment of linear features between adjacent planes is not achieved. \wdx{Note we here choose a zoom-in view with the most obvious misalignment among given buildings to clearly show this issue. The other examples may also exhibit tiny misalignments.}
Third, we may fail to successfully perform inpainting for a reflected facade which lacks of coherent structures and clear content, making it even hard for a human to infer the missing region, see Fig.~\ref{fig:limitations} (right).
Finally, the processing time can be further improved with parallel processing. We will incorporate these issues in our future pipeline.



==> src/backup/old-src/01-intro.tex <==
\section{Introduction}\label{sec:intro}

Automatic 3D reconstruction of large-scale urban environments has experienced an increasing interest in computer graphics and compute vision communities. With the advances in active sensors (\eg LiDAR) and fully automated \emph{Multiple View Stereo} (MVS), many mature algorithms have been developed to generate complete and high-fidelity 3D geometry models~\cite{musialski2013survey}. Especially the recent aerial-based photogrammetry sensing technology achieves the generation of city-scale surface models from aerial oblique images, which are also enriched with high resolution textures~\cite{Smith2018Aerial,Hepp2018Plan3D,zhou2020offsite}. %,Liu2021Aerial,zhang2021continuous}. 

Although yielding impressive 3D reconstruction, all of these methods generate triangular meshes containing a huge amount of details. Such a dense mesh is a very redundant 3D representation and also lacks high-level semantic and structural information. The direct use of such meshes is often intractable in practical applications, for example, causing a lot of burden on model storage,  transmission, editing and real-time rendering. Therefore, there is rising attention to transforming dense meshes into simplified and concise polygonal models by either geometry simplification/approximation~\cite{garland1997surface,cohen2004variational,salinas2015structure} or structure-aware surface reconstruction~\cite{verdie2015lod,kelly2017bigsur,bauchet2020kinetic,bouzas2020structure}. 

Although achieving compact and plausible coarse models, these methods focus only on geometry and mostly ignore appearance aspects, \ie the texture information contained in the original mesh is not maintained. In practice, manually creating high-quality textures is often required for increasing the reality of urban environments, but it is quite tedious and time consuming. %authoring realistic urban environments
Another intuitive way is to directly applying existing facet-based texture generation methods~\cite{lempitsky2007seamless,waechter2014let,zhou2014color} on the coarse mesh. However, these approaches would produce distorted and misaligned artifacts as illustrated in Fig.~\ref{fig:facet-based}, due to i) the significant geometric differences between the simplified mesh and ground-truth models, and ii) the inaccurate estimated camera extrinsic parameters. Moreover, the structured urban buildings usually have obvious large-scale planar structures, \eg a large plane is represented by only two triangular faces. 
For such planes, in the view selection step, previous approaches may not find a suitable image that contains all the texture information for a large triangular face, leading to this triangular face untextured.

Motivated by the above issues, we focus on the problem of texture generation for structured building models. In contrast to all previous works, we propose a new plane-based texture generation method based on image stitching, which can automatically generate photo-level textures for a simplified mesh. 
First, we should solve how to select a minimum set of views that are most suitable for texturing the corresponding planar region of the simplified mesh, and then denote the most representative view as reference view. Second, we warp images from other views to the reference view by preserving important geometric primitives and stitch the visible region of the plane in the image space into an enlarged texture map. Finally, the texture is optimized to generate a high-quality texture for each plane.

Experimental results demonstrate that the quality of texture maps generated by our plane-based texture generation method surpasses that of the facet-based methods. Besides, our approach achieves competitive results in terms of quality and compactness compared with texture maps manually produced by a human-expert in much less time.  

\begin{figure}[tp]
    \centering
    \includegraphics[width=0.6\linewidth]{figs/facet_base.pdf}
    \caption{Two issues of facet-based texture generation method~\cite{waechter2014let}. First, important geometric primitives such as line-segments are not well preserved in the texture map (right-top). Second, visible seams exist along the border edge between two large facets (right-bottom).}
    \label{fig:facet-based}
\end{figure}

% Although a high-quality texture
% map can be easily computed for accurate geometry and calibrated cameras,
% the quality of texture map degrades signifcantly in the presence of inaccuracies.

% Therefore, naïvely projecting
% and combining the input images produces blurring and ghosting
% artifacts, as shown in Fig. 2.

% Inspired by the recent success of patch-based methods in image
% and video editing tasks, we propose a novel global patch-based opti-
% mization system to synthesize aligned images.



% Manually creating high-quality textures is time consuming
% – not only must the details of the textures match the ge-
% ometry, but stylistic consistency both within single struc-
% tures and between adjacent structures or their surroundings
% (e.g. between buildings, street-furniture, and sidewalks) is
% also required.

% Our goal is to process 3D meshes to create
% texture maps which are detailed, fit the geometry, and are
% free from local or global discontinuities.



% However, producing photorealistic models of real-world
% environments requires not only geometric reconstruction
% but also high-quality color texturing. Unfortunately, due
% to noisy input data, poorly estimated surface geometry,
% misaligned camera poses, unmodeled optical distortions,
% and view-dependent lighting effects, aggregating multiple
% real-world images into high-quality, realistic surface tex-
% tures is still a challenging problem.

% On the other hand, 3D models have
% rich full-object geometry, but often lack realistic textures needed
% for high-quality renderings. 


% Texture mapping plays an important role in reconstructing virtual versions of
% real-life products for E-Commerce applications with inexpensive consumer-grade
% scanning devices. This raises challenging problems to reconstruct seamless, high-
% quality texture maps from noisy data, such as inaccurate geometry, imprecise
% camera poses, and optical distortions of consumer-grade cameras.

% Geometry reconstruction has been the subject of extensive
% research and many powerful algorithms have been developed [Seitz
% et al . 2006]. With the availability of consumer depth cameras to the
% public, ordinary users are now able to produce geometric models of
% objects using techniques like KinectFusion [Newcombe et al . 2011].
% However, reproducing the full appearance of real-world objects
% also requires reconstructing high-quality texture maps.



% 3D reconstruction techniques can recover textures by extracting corresponding texture patches from multiple views and
% mapping them onto the reconstructed 3D meshes. But the recovered texture patches may not be perfectly aligned on the
% reconstructed 3D meshes due to the unavoidable errors in both camera calibration and geometry reconstruction. Moreover
% varied luminance and scale between different views in large-scale datasets make it to recover photo-realistic textured mod-
% els free of artifacts.


==> src/backup/old-src/02-rw.tex <==
\section{Related Work}\label{sec:rw}

\subsection{Image-based Texture Mapping}

Texture mapping is an important approach for authoring photo-realistic 3D objects without increasing their geometric complexity~\cite{yuksel2019rethinking}.
Early works on image-based texture mapping usually select multiple images for each face and blend them into textures by using different weighting strategies~\cite{bernardini2001high,callieri2008masked}. However, such blending-based methods could generate blurry and ghosting results due to camera calibration errors and inaccurate geometry. 
To reduce those artifacts caused by multi-image blending, many projection-based approaches~\cite{lempitsky2007seamless,wang2018seamless,gal2010seamless,waechter2014let,fu2020joint} are proposed to improve the effect of texture mapping. This kind of method first select only one view per face to create a texture patch, then conduct seam optimization to avoid visible seams between adjacent texture patches. 
To jointly rectify the camera poses and geometric errors, Zhou and Koltun~\shortcite{zhou2014color} use local image warping to optimize camera poses in tandem with non-rigid correction functions for all images. This approach is then extended to handle larger geometry inaccuracies~\cite{fu2018texture,bi2017patch}. However, all of above previous methods directly map the color information of high-resolution images to the 3D mesh, and the result of texture mapping greatly depends on the 3D reconstruction quality. Therefore, non of them can be naively applied to a structured model, which has significant structural differences from the original dense mesh. Furthermore, they all fail to align large-scale geometric features, resulting in obvious seams in the generated texture maps. 

\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/pipeline.pdf}
    \vspace{-0.5cm}
    \caption{Overview of our algorithm. Taking a structured mesh and the UAV images as input, our system detects the boundary polygon and generates one stitched texture map for each planar region in the mesh. Firstly, a minimum subset of views are selected from all the visible views for each planar shape. Secondly, all the selected views are stitched together to form an enlarged texture map. Note that important geometric primitives such as line-segments contained in the original images are well preserved after the image stitching. Finally, the texture map is optimized by performing global consistency across all the visible region and image paining on the invisible region of the underlying planar shape.}
    \label{fig:pipeline}
\end{figure*}

% Although high-quality texture maps can be generated from above methods, 
% easily computed for accurate geometry and calibrated cameras, the quality of texture map degrades signifcantly in the presence of inaccuracies.

\subsection{Structure-aware Scene Reconstruction and Texturing}

Creating concise and structured polygonal models from noisy raw data has become an ever-increasing demand in urban reconstruction. A popular approach is to first reconstruct a dense mesh then simplify it using geometry simplification~\cite{garland1997surface} or piecewise-planar structure approximation methods~\cite{cohen2004variational,verdie2015lod,salinas2015structure}. Another kind of methods detect a set of planar primitives from the point clouds, then explore the arrangements of primitives to provide a compact polygonal mesh~\cite{Monszpart2015rapter,Nan2017polyfit,fang2020connect,bauchet2020kinetic,bouzas2020structure,Pan2022Efficient}.
In our approach, we utilize an efficient and robust structure-aware surface reconstruction~\cite{Pan2022Efficient} to generate the simplified meshes from point clouds or raw triangular meshes.

Texturing simplified meshes or coarse building models has drawn less attention. Several methods take into account the generation of texture maps while conducting a lightweight geometric reconstruction~\cite{garcia2013automatic,huang20173dlite,maier2017intrinsic3d,wang2018plane}. For example,~\cite{garcia2013automatic} compute a per-building volumetric proxy, then use a surface graph cut method to stitch aerial images and yield a visually coherent texture map. However, their reconstruction results are 2.5D which can only restore textures under a limited perspectives, resulting in the generated textures losing many important structures. 
Aiming at indoor scene reconstruction, 3DLite~\cite{huang20173dlite} presents a primitive-based scene abstraction, then uses the planar-based constraint to generate high-quality textures on abstracted geometry through texture optimization. 
Due to a lot of assumptions are made for the structure of the indoor scene and too many texture loss functions to be optimized, the generalization of this method is limited and its convergence speed is slow. 
Recently, deep learning approaches based on image-image translation networks have been proposed to synthesize texture details for coarse building meshes of urban areas~\cite{Kelly2018FrankenGAN,georgiou2021projective}. 
Although these methods are able to generate various styles of textures, they require extensive training set and the synthesized textures may lack realism compared to the original real scenes.

\subsection{Image Stitching and Completion}
Another class of work most relevant to ours is image stitching, which combines multiple images with overlapping sections to produce a single panoramic or high-resolution image~\cite{szeliski2007image,Mehta2011}.  
%is a central and long-studied problem in computer graphics~\cite{szeliski2007image,Mehta2011}.
Early methods estimate an optimal global transformation for each input image~\cite{brown2007automatic}. However, they only work well for scenes that are near planar or with slight view disparity, and usually generate ghosting artifacts or projective distortion for general scenes. 
For more accurate stitching, many approaches adopt spatially-varying warps to process different regions of an image, including smoothly varying affine transformation~\cite{lin2011smoothly}, dual or quasi homographies~\cite{gao2011constructing,li2017quasi}, shape-preserving half-projective warps~\cite{chang2014shape,lin2015adaptive}, and smoothly varying homography field~\cite{zaragoza2013projective}, etc. 
However, they are usually time-consuming and not suitable for scenes with large parallax. Several methods are then proposed to obtain better alignment with less distortion especially for large parallax~\cite{zhang2016multi,lee2020warping}, but linear structures in the image are not well maintained. After that, instead of just using point feature matching, line features are introduced to preserve both linear structures~\cite{li2015dual,xiang2018image,liao2019single,jia2021leveraging}. 
All these methods apply an uniform grid to warp the images, which are not flexible enough to align the regions with dense geometric features. Unlike them, we propose to use an adaptive grid to locally warp the images and better align the large-scale line features.
% ~\cite{li2017parallax}
% ~\cite{herrmann2018robust}
%~\cite{chen2016natural}
%~\cite{lin2017direct}
%~\cite{zhang2014parallax}
%~\cite{lin2016seagull}

Image completion, also known as image inpainting, is the process of restoring missing or damaged areas in an image. Extensive research has been conducted on image completion, and existing methods can be classified into three types: 1) diffusion-based methods, 2) patch-based methods and 3) deep learning methods based on generative models. A detailed review is out of the scope of the paper, and we refer the reader to recent surveys~\cite{guillemot2014image,rojas2020a,elharrouss2020image,jam2021a}. 



==> src/backup/old-src/03-overview.tex <==
\section{Problem Statement and Overview}
\label{sec:overview}

The objective of our approach is to automatically generate seamless and structure-aware texture maps for man-made objects composed of piecewise-planar shapes, \ie urban buildings. Our algorithm takes a structured model $\mathcal{M=(E, F)}$ and a set of calibrated camera views $\mathcal{V=(I, T, K)}$ as input, and outputs a set of compact texture maps. To be precise, $\mathcal{M}$ is a polygonal mesh where each basic element of $\mathcal{F}$ is either a polygonal or a triangular facet returned by structure-aware surface reconstruction methods ~\cite{verdie2015lod,kelly2017bigsur,fang2020connect,bauchet2020kinetic,bouzas2020structure}. \jwc{define the planar shape $\mathcal{M}_i \subset \mathcal{M}$}
The tuple of $\mathcal{(I, T, K)}$ represents the collected images, extrinsic and intrinsic camera parameters. Since each urban building is considered as an assembly of planar shapes, directly applying previous methods to select the best view for each facet can not guarantee that most part of each planar region is textured by only few number of image patches. Moreover, visible seams occurred at the boundary of adjacent patches damage the quality of final texture maps. 

\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/view_selection.pdf}
    \vspace{-0.5cm}
    \caption{Illustration of our view selection process. At each iteration, for each planar shape, the candidate view with maximum gain of information (denoted by $G$) is selected. Moreover, the total observed region of current planar shape is updated as the union part of all the observed region of previously selected views (red polygons), and \red{the gain of information as well as visible region of each view (blue polygons) are recomputed.}}
    \label{fig:view_selection}
\end{figure*}

In this work, we propose a plane-based texture generation approach to provide one enlarged seamless texture map for each planar shape of the building surface. Fig.~\ref{fig:pipeline} illustrates the pipeline of our algorithm, which consists of three main steps. %Three main steps are involved in our method. 
First, in Sec.~\ref{sec:view selection}, we select a minimum set of views that are most suitable for texturing and best cover each planar shape contained in the structured mesh. Among these selected views, the most representative view is determined as the reference image and all the other views are considered as target images. Second, in Sec.~\ref{sec:image stitching}, all the target images are warped to the reference image by detecting and aligning line-segments contained in the original images. Moreover, we propose an adaptive mesh data-structure to perform the image warping operator while preserving the straightness and completeness of the extracted line-segments. In this step, we obtain one single enlarged image by stitching each visible region of current planar shape contained in each view serving as the texture map for the underlying plane. Finally, in Sec.~\ref{sec:texture optimization} each texture map is adjusted to a virtual view that can best visualize the corresponding planar region and then optimized by a series of operators to reveal global perceptual consistency.
 
% The goal of most image-based texture mapping approaches is to pro-
% duce a high-quality view-independent texture map using a set of N
% source images, S 1 ,··· ,S N , taken from different viewpoints. These
% methods usually assume that the object’s approximate geometry
% and rough camera poses (i.e., extrinsic and intrinsic parameters)
% of all the source images are already estimated using existing tech-
% niques [Newcombe et al . 2011; Seitz et al . 2006]. Once the texture
% map is created, the object with a view-independent texture can be
% rendered from any novel views.

% Texture mapping is a standard tech-
% nique widely used with meshes. Here, surface appearance is
% represented by a 2D texture image and a 3D-to-2D mapping
% from every mesh vertex to the texture space. Textures can
% be easily controlled and edited by artists as needed to create diversities of scene appearance.


% Texturing a 3D model from multiple registered images is typically performed in
% a two step approach: First, one needs to select which view(s) should be used to
% texture each face yielding a preliminary texture. In the second step, this texture
% is optimized for consistency to avoid seams between adjacent texture patches.


% Texture mapping methods for
% large-scale scenes mainly consist of two steps: 1. view selection in order to select different views to create a texture patch
% for each face. 2. seam optimization which is applied to eliminate visible seams among the borders of texture patches. They
% can be classified into two different categories according to their view selection strategies.

==> src/backup/old-src/04-method.tex <==

\begin{figure}[tp]
    \centering
    \includegraphics[width=0.75\linewidth]{figs/plane_extraction.pdf}
    \vspace{-0.5cm}
    \caption{Planar shape boundary extraction. All facets of input mesh is first segmented into different planar regions and the boundary polygons are then extracted for each planar shape. \jwc{what are the boundary polygons?}}
    \label{fig:boundary_extraction}
\end{figure}

\section{Plane-based Texture Generation}
\label{sec:method}

%In this section, we present in detail three main phases involved in our plane-based texture generation approach.

%Directly apply previous triangular-facet based texture mapping methods to such data leads to inevitable mistakes as shown in Figure \ref{}. Thus, we proposed a plane-based texture mapping approach to handle those issues. 


%In this section, we describe our texture mapping method based on planar structure for large-scale urban building. We extract planes and polygons from structured mesh (Section 4.1). These geometry structures will be used as the basic unit in view selection stage (Section 4.2). Finally a line preserved image stitching method will combine the patches from different views into a complete texture for each plane.

%\subsection{Plane Extraction}

%Since the structured urban buildings usually have obvious large-scale planar structures, we can easily extract the planes $P$ by using region growing. We then extract the borders of the planes by searching the common edge of two planes. For each plane we traverse along its borders and save the common points $p$ when the angle between two edges not equal to $\pi$. 

% \newpage

\subsection{View Selection} \label{sec:view selection}
The objective of this step is selecting a minimum subset of camera views as the candidate feature maps for each planar shape $\mathcal{M}_i \subset \mathcal{M}$. To achieve this goal, we first detect the \red{supporting plane} for each planar shape $\mathcal{M}_i$ by utilizing a region growing algorithm and extract the corresponding boundary polygons $\mathcal{P}_i$ by choosing and sorting the boundary edges of $\mathcal{M}_i$. Note that some planar shapes which are composed of nested polygons are also taken into account in our algorithm as shown in Fig.~\ref{fig:boundary_extraction} \jwc{what are the nested polygons?}.

Next, we determine the set of candidate valid views $\mathcal{I}_i \subset \mathcal{I}$ by checking the visibility between each camera view and planar shape $\mathcal{M}_i$ as well as the photo-consistency. In particular, a camera view is considered as valid if the following criteria are satisfied:
\begin{itemize}[leftmargin=*]
    \item The camera position should locate in front of the planar shape.
    \item The observation angle between the view direction and the normal vector of planar shape should be smaller \revise{than a threshold $\theta$ ($\theta=75^{\circ}$ in default)}.
    \item The projection area of boundary polygons $\mathcal{P}_i$ on the corresponding image should be larger than zero.
    \item There is no occlusion occurred between the camera view and planar shape, which can be determined by computing the intersections between each facet of planar shape $\mathcal{M}_i$ and viewing rays from camera origin to the center of facet.
\end{itemize}

After that, we perform a photo-consistency checking using the method proposed in \cite{waechter2014let} and consider the camera views exhibiting distinctive illuminance against other views as outliers. All the outlier views are filtered from $\mathcal{I}_i$ and we obtain the potential candidate camera views for texturing boundary polygons $\mathcal{P}_i$. However, it is not an optimal solution to utilize all the remaining views to generate texture maps due to the following concerns. First, some part of $\mathcal{P}_i$ can be observed by several candidate views and employing all of these views to texture the overlapping regions inevitably produces significant seams at the region border. Second, each candidate view promotes different contributions while texturing the planar shape under question considering the visible region area of $\mathcal{P}_i$ on image, view proximity and angle. Third, each view reveals various distributions of colors and makes it difficult for the downstream steps to optimization the texture maps to improve the global photo-consistency. \jwc{I can not understand the last two reasons.}

To handle the above issues, we propose a submodular optimization formalism to search an optimal minimum subset of views $\mathcal{\hat{I}}_i \subset \mathcal{I}_i$ as the final selected views formulated by
\begin{equation}
    \mathcal{\hat{I}}_i=\mathop{\arg\max}\limits_{\mathcal{I}^{*}_{i} \in P(\mathcal{I}_i)}{E(\mathcal{I}^{*}_{i})} \text{,}
\end{equation}
where $P(\mathcal{I}_i)$ denotes the power of candidate views \jwc{What is the power of candidate views?} $\mathcal{I}_i$ and the objective function $E(\mathcal{I}^{*}_{i})$ measures the amount of information that all the selected views in $\mathcal{I}^{*}_{i}$ contribute to texturing the underlying planar shape $\mathcal{M}_i$ in form of
\begin{equation}
E(\mathcal{I}^{*}_{i})=\sum_{\mathcal{I}^{j}_{i} \in \mathcal{I}^{*}_{i}}{G(\mathcal{I}^{j}_{i}, \mathcal{M}_i)} \text{,}
\end{equation}
where $G(\mathcal{I}^{j}_{i},\mathcal{M}_i)$ estimates the gain of information to observe and texture $\mathcal{M}_i$ provided by current view $\mathcal{I}^{j}_{i}$. Note that such formulation guarantees the submodularity of objective function since the newly inserted view will not reduce the total information. Therefore, we can rely on a greedy algorithm to approximately select the best subset of views without the issue of non-convergence. Typically, at each iteration $t$, we update $\mathcal{\hat{I}}_i^{t}=\{\mathcal{\hat{I}}^{j}_{i}\}\cup{\mathcal{\hat{I}}_i^{t-1}}$, where $\mathcal{\hat{I}}^{j}_{i}$ is the candidate view with the largest gain of information computed as 
\red{
\begin{equation}
G(\mathcal{I}^{j}_{i}, \mathcal{M}^{t}_{i})=D(\mathcal{I}^{j}_{i}, \mathcal{M}^{t}_{i})\cdot C(\mathcal{I}^{j}_{i}, \mathcal{M}^{t}_{i}) \cdot N(\mathcal{I}^{j}_{i}, \mathcal{M}^{t}_{i}) \text{,}
\end{equation}
}
where $\mathcal{M}^{t}_{i}$ denotes the unobserved region of $\mathcal{M}_{i}$ by any of the selected views until iteration $t-1$. In particular, this region is updated by $\mathcal{M}^{t}_{i}=\mathcal{M}^{t-1}_{i}\setminus~\mathcal{R}^{t-1}_{i}$, where $\mathcal{R}^{t-1}_{i}$ is the visible region of $\mathcal{P}_i$ on the selected image $\mathcal{\hat{I}}^{j}_{i}$ at iteration $t-1$, which can be extracted by computing the intersection polygons between visible region of $\mathcal{P}_i$ on  $\mathcal{\hat{I}}^{j}_{i}$ and the boundary polygon of $\mathcal{\hat{I}}^{j}_{i}$. Besides, $D(\mathcal{I}^{j}_{i}, \mathcal{M}^{t}_{i})$ measures the sum of the gradient magnitude over all pixels within the projection region as the method introduced in~\cite{gal2010seamless}. This term favors large projection region revealing that the camera is close to the underlying planar shape. $C(\mathcal{I}^{j}_{i}, \mathcal{M}^{t}_{i}))$ exhibits the photo-consistency of $\mathcal{I}^{j}_{i}$ against the other candidate images in region $\mathcal{M}^{t}_{i}$. This term is computed by a multi-variate Gaussian function as the method proposed in~\cite{waechter2014let}. $N(\mathcal{I}^{j}_{i}, \mathcal{M}^{t}_{i})$ denotes the normal deviation between the viewing ray from camera origin to the center of $\mathcal{M}^{t}_{i}$ and the normal vector of $\mathcal{M}_{i}$, which favors front-parallel views. Our greedy algorithm stops until the whole region of $\mathcal{M}_{i}$ is observed by selected views $\mathcal{\hat{I}}_i^{t} \subset \mathcal{I}_i$ or the largest area of visible region of $\mathcal{M}^{t}_{i}$ on the remaining images $\mathcal{I}_i \setminus \mathcal{\hat{I}}_i^{t}$ is smaller than a threshold $\alpha=0.05$. Fig.~\ref{fig:view_selection} illustrates this greedy view selection mechanism. 

\subsection{Image Stitching} \label{sec:image stitching}
For each planar shape $\mathcal{M}_i$ surrounded by boundary polygons $\mathcal{P}_i$, we obtain a minimum subset of camera views $\mathcal{\hat{I}}_i$ to generate texture maps. One intuitive solution is to extract texture patches from $\mathcal{\hat{I}}_i$ for each part of $\mathcal{P}_i$ as previous method \cite{waechter2014let}. However, such strategy suffers from two obstacles. First, the corresponding extrinsic parameters are not perfectly accurate which cause obvious seams at the borders of texture patches. Second, important geometric priors such as boundary edges in texture maps are not explicitly extracted and preserved across adjacent patches. Therefore, we propose a plane-based image stitching mechanism to generate one complete texture map for $\mathcal{P}_i$ by aligning the line-segments detected in each image during the warping procedure. In our algorithm, we consider the first selected image in $\mathcal{\hat{I}}_i$ as a reference image and the other images as target images, then all the target images are warped to the reference image by the order of their insertion into $\mathcal{\hat{I}}_i$.

% \begin{figure}[tp]
%     \centering
%     \includegraphics[width=\linewidth]{figs/adaptive_mesh.pdf}
%     \vspace{-0.5cm}
%     \caption{test2}
%     \label{fig:pre-alignment}
% \end{figure}

For each target image $\mathcal{I}^{tar}$, we first estimate the homography relationship between itself and reference image $\mathcal{I}^{ref}$. In our problem, the whole region of $\mathcal{P}_i$ is coplanar and the local homography perfectly holds inside the planar shape region. One solution is to directly compute the homography matrix $\mathcal{H}_{tar}^{ref}$ as a composition of the camera parameters $(\mathcal{K}^{tar}, \mathcal{K}^{ref}, \mathcal{T}^{tar}, \mathcal{T}^{ref})$. However, this strategy can not avoid the misalignment caused by slightly inaccurate camera parameters. We instead back project each vertices of $\mathcal{P}_i$ on both $\mathcal{I}^{ref}$ and $\mathcal{I}^{tar}$, and then compute $\mathcal{H}_{tar}^{ref}$ by solving $p_i^{ref}=\mathcal{H}_{tar}^{ref}\cdot p_i^{tar}$,
where $p_i^{ref}$ and $p_i^{tar}$ denote the back projection pixel positions of vertices of $\mathcal{P}_i$ on $\mathcal{I}^{ref}$ and $\mathcal{I}^{tar}$ respectively. Although this rough result provides a relatively accurate transformation from $\mathcal{I}^{tar}$ to $\mathcal{I}^{ref}$, the important geometric structures are not well preserved and causes visible distortion after the warping as show in Fig~\ref{fig:pre-alignment}.

Hence, we employ the traditional LSD algorithm \cite{LSD} to detect line-segments from the visible region of $\mathcal{P}_i$ on $\mathcal{I}^{tar}$ and $\mathcal{I}^{ref}$, which are denoted as $\mathcal{L}^{tar}$ and $\mathcal{L}^{ref}$ respectively. These two initial sets of line-segments are refined by merging close and collinear segments. We then find the matching relationship between two set of line-segments. Since all of the line-segments in $\mathcal{L}^{tar}$ and $\mathcal{L}^{ref}$ locate inside $\mathcal{P}_i$, the pre-estimated homography relationship $\mathcal{H}_{tar}^{ref}$ still holds. Therefore, we transform $\mathcal{L}^{tar}$ to reference image and obtain warped line-segments $\mathcal{\overline{L}}^{tar}=\mathcal{H}_{tar}^{ref}\cdot \mathcal{L}^{tar}$. For each line-segment $\overline{l}^{tar} \in \mathcal{\overline{L}}^{tar}$, it is registered to line-segment $l^{ref} \in \mathcal{L}^{ref}$ if the angle between two supporting lines is smaller than $5^{\circ}$ and the maximum point-two-line distance from four end-points to another line is closer than 3 pixels. We denote $\mathcal{L}$ as the set of all pairs of matched line-segments between $\overline{\mathcal{L}}^{tar}$ and $\mathcal{L}^{ref}$.

\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/pre-alignment.pdf}
    \vspace{-0.5cm}
    \caption{Pre-alignment. The warping relationship from target image to reference image can be easily determined by computing the homography matrix between the corresponding projection vertices of $\mathcal{P}_i$ (red polygons) on two images. However, simply stitching target image with reference image produce geometric inconsistency across their boundaries.}
    \label{fig:pre-alignment}
\end{figure}

We next warp $\mathcal{I}^{tar}$ to $\mathcal{I}^{ref}$ while preserving the matched line-segments of $\mathcal{L}^{tar}$. Previous work proposed in \cite{jia2021leveraging} converts the rigid transformation into a global line-guided mesh deformation problem. They rely on deforming the vertices of a grid-mesh uniformly sampled in the target image to maintain line structures by solving a global least-square energy function. However, the global optimal deformation results do not guarantee the strict straightness of line-segments. There, we propose an adaptive-mesh data structure to explicitly maintain the line-segments after warping. To be precise, the target image is initially transformed to $\mathcal{\overline{\mathcal{I}}}^{tar}=\mathcal{H}_{tar}^{ref}\cdot \mathcal{I}^{tar}$ and we insert all the edges of boundary polygons $\mathcal{P}_i$ as well as the line-segments in $\overline{\mathcal{L}}^{tar}$ into the 2D domain. We next construct a constrained Delaunay triangulation $M^{tar}=(V^{tar},E^{tar},F^{tar})$, keeping all the inserted segments as constraint edges. Unlike previous uniformly sampling grid-mesh data structure, every basic element in our adaptive mesh encodes a meaningful geometric primitive in the target image, \ie a corner point or a line-segment as demonstrated in Fig.~\ref{fig:adaptive_mesh}. Based on this, all the vertices $V^{tar}$ are deformed to new positions $\widetilde{V}^{tar}$ while satisfying the following two constraints:
\begin{itemize}[leftmargin=*]
    \item The matched line-segment pairs in $\mathcal{L}$ are well aligned after the mesh deforming.
    \item All the line-segments in $\overline{\mathcal{L}}^{tar}$ preserve straightness after the mesh deforming.
\end{itemize}
We search for the optimal deformation offset $\Delta{V}=\widetilde{V}^{tar}-V^{tar}$ by embedding these two requirements into the following energy minimization formulation: 
\begin{equation}
    E(\Delta{V})=\lambda~E_a(\Delta{V})+E_l(\Delta{V}) \text{.}
\end{equation}
%where the offset of vertices is represented by \[\Delta{V}=[\Delta{V_{1x}},\Delta{V_{1y}},\Delta{V_{2x}},\Delta{V_{2y}},\ldots]^{T}\] 
 $E_a(\Delta{V})$ encodes the line-alignment term, which guarantees the alignment between all pairs of matching line-segments in $\mathcal{L}$ after deforming vertices by $\Delta{V}$ in form of
\begin{equation}
    E_a(\Delta{V}) = \sum_{t=1}^{|\mathcal{L}|}d(V^{tar}_{t1}+\Delta{V_{t1}}, l_t^{ref})+ d(V^{tar}_{t2}+\Delta{V_{t2}}, l_t^{ref}) \text{,}
\end{equation}
where $l_t^{ref}$ is the $t-$th matched line-segment in $\mathcal{L}^{ref}$, and $(V^{tar}_{t1},V^{tar}_{t2})$ are end points of $t-$th matched line-segment in $\overline{\mathcal{L}}^{tar}$. Moreover, the line-preserving term denoted as $E_l(\Delta{V})$ ensures the straightness of each line-segment in $\overline{\mathcal{L}}^{tar}$ after mesh deformation by
\begin{equation}
    E_l(\Delta{V}) =\sum_{j=1}^{|\overline{\mathcal{L}}^{tar}|} [(V^{tar}_{j1}+\Delta{V_{j1})-(V^{tar}_{j2}+\Delta{V_{j2})}^T \cdot \overrightarrow{n}_j^{tar}} \text{,}
\end{equation}
where $(V^{tar}_{j1},V^{tar}_{j2})$ are end points of $j$-th line-segment $l_j^{tar}$ in $\overline{\mathcal{L}}^{tar}$ and $\overrightarrow{n}_j^{tar}$ is the normal vector of $l_j^{tar}$. $\lambda$ is set to 0.5 in our experiments. The optimal offset is then solved by conjugate gradient algorithm. Finally, each pixel $p^{tar}$ inside the adaptive mesh facet $f\in F^{tar}$ is warped to the new position $\widetilde{p}^{tar}$ by performing an affine transformation constructed by the offset of the three incident vertices of $f$. Until now, all the visible region of target image is warped to $\mathcal{I}^{ref}$ and form an enlarged reference image to use.

\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/adaptive_mesh.pdf}
    \vspace{-0.5cm}
    \caption{Adaptive mesh data-structure. We construct a constrained Delaunay triangulation by inserting detected line-segments and edges of boundary polygons as constraints.}
    \label{fig:adaptive_mesh}
\end{figure}

\subsection{Texture Optimization} \label{sec:texture optimization}
Previous step enables us to generate a whole texture map $\mathcal{I}^{ref}$ for each planar shape $\mathcal{M}_i$. This step aims at improving the quality of $\mathcal{I}^{ref}$ relying upon a series of texture optimization operators.


First, to visualize $\mathcal{M}_i$ in a fronto-parallel view, we adjust $\mathcal{I}^{ref}$ to a new viewing point and place a virtual camera with extrinsic parameters $\mathcal{T}^{vir}=[\mathcal{R}^{vir}, t^{vir}]$. The viewing direction of the virtual camera is $-\overrightarrow{n_i}$, the reverse direction of the normal vector of $\mathcal{M}_i$. Thus we get $\mathcal{R}^{vir}=\mathcal{R}(\overrightarrow{n_i})^T$, where $\mathcal{R}(\overrightarrow{n_i})$ represents the rotation matrix extended by $\overrightarrow{n_i}$. The virtual camera is translated from the center $\mathcal{C}_i$ of $\mathcal{M}_i$ along the direction $\overrightarrow{n_i}$ with a distance $d$ until %he whole region of 
$\mathcal{M}_i$ is covered in the virtual image, and the translation vector $t^{vir}=-\mathcal{R}(\overrightarrow{n_i})\cdot(\mathcal{C}_i+\overrightarrow{n_i}d)$. After finding the best viewing point, $\mathcal{I}^{ref}$ is warped to $\mathcal{I}^{vir}$ by computing their homography matrix.

Next, since the new texture map $\mathcal{I}^{vir}$ is composed by patches extracted from various views, the global brightness would not be consistent across patches due to different viewing directions. Thus, we perform a global illumination consistency on $\mathcal{I}^{vir}$ under the assumption that the distribution of brightness over the whole texture map holds a similar pattern. To achieve this goal, we adjust the brightness of non-overlapping region contributed by target image guided by the brightness of the overlapping region between itself and reference image. To be precise, we transfer selected views to HSV color space and calculate a distribution histogram of value ($V$, last channel of HSV) on non-overlapping region of target image and overlapping region on reference image respectively. Next, we match these two histograms and transfer the brightness of overlapping region on reference image to non-overlapping region on target image by performing a look-up table transform of the histogram matching results.

\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/texture_optimization.pdf}
    \vspace{-0.5cm}
    \caption{Texture optimization. The enlarged textured map is optimized by global illumination consistency and line-guided inpainting operators.}
    \label{fig:texture_optimization}
\end{figure}

In practice, some part of each planar shape would not be observed by any of the selected view. Thus, the final step of our algorithm aims at inpaining the texture map $\mathcal{I}^{vir}$ for each planar shape. Inspired by linear geometric features based image completion method proposed in~\cite{huang2014image}, we employ a similar approach to inpaint the missing parts of each plane. Unlike their method that detects three main direction planes from three vanishing points under Manhattan-World assumption, our texture map exhibits only one planar shape. Thus, we instead detect two set of parallel line-segments and utilize these regularity to guide the image painting using the propagation mechanism in Patch  Match~\cite{barnes2009patchmatch}. Finally, we perform Poisson-Image-Editing~\cite{perez2003poisson} to eliminate the seams at the borders of inpainting region.

%(1) Texture shrink.

%Due to the different selection of viewing point, to keep the image resolution, we sometimes get images with large resolution but less image information, which makes it difficult for our later rendering. Therefore, for each plane, we zoom in and out the image by a certain factor multiple times and compare it with the original image until the error per pixel is greater than 0.5%. The size of the plane can be effectively reduced without losing the main information.

%(2) Illumination consistency

% In our method, texture is composed by patches from multi views for each plane. Due to the difference of the illumination between views, the patches in same plane will have different brightness, which cause significant artifact. 

%(3) Texture inpainting

%Sometimes, due to the lack of perspective, the plane we get is not complete all the time. Therefore, we need to fill the missing part according to the information from plane itself. In recent related work, most of the missing areas are processed using the Encode-Decode structure of machine learning algorithms. However, our testing found that the generalizability of these methods is dependent on their dataset. At the same time, due to the limitation of hardware, these methods can usually only process images with a maximum size of 512*512. And our single plane may have a maximum size of 5000*5000 depending on the viewing point we choose, because the information that needs to be completed in each picture is basically included in the picture, based on the idea of Patch Match, and we follow the work of [Huang et al. 2014], method as our main method for completion.

%According to Huang et al., they use the linear feature-guided method as the search index of the image, but at the same time we note that the paper assumes that there are 3 vanishing points in the image according to the large number of man-made buildings in the image , every two pairs constitute a plane represented by an vanishing line to guide the area to be filled. And then, our simplified model has kept only one single plane, most of which are parallel lines, this assumption obviously does not apply to our processing logic. Therefore, we changed the vanishing points that need to be clustered to two.







==> src/backup/old-src/05-results.tex <==
\section{Experimental Results}\label{sec:results}

To validate the proposed algorithm, we start with a series of experiments on real-world scenes with complex structures of varying styles. 
Then we evaluate our approach qualitatively and quantitatively by comparing against state-of-the-art texture generation approaches and human-experts. Finally, we demonstrate the main technical ingredient effectiveness by ablation studies.
Our algorithm is implemented in C++, and all the experimental results presented in this paper are obtained on a desktop computer equipped with an Intel i7-7700k processor with 4.2 GHz and 32 GB RAM.

\begin{figure*}[!th]
    \centering
    \includegraphics[width=\textwidth]{figs/L7_compare.png}
    \caption{Visual comparison against RC on scene Polytech, where the detailed comparisons are shown in the zoomed-in insets.}
    \label{fig:cmp_rc}
\end{figure*}

\noindent\textbf{Dataset.}
For our performance evaluation and comparisons, we carry out experiments on real-world scenes, either from public sources (e.g., Library~\cite{zhang2021continuous}, Hitech~\cite{zhou2020offsite}, Polytech and ArtSci~\cite{liu2021urbanscene3d}) or captured by a single-camera drone (\eg Mobile, Sunshine Plaza, Hall). 
Then we use the commercial software RealityCapture~\footnote{https://www.capturingreality.com/} to reconstruct the 3D high-precision models from the captured images. Finally, we employ structure-aware surface reconstruction method proposed in~\cite{bauchet2020kinetic} to generate the simplified coarse models. All of the dense and coarse models are utilized to demonstrate the performance of our algorithm throughout whole experiments.

\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/manual.png}
    \caption{Comparison on scene Mobile and Hitech with manual texturing mechanism.}
    \label{fig:cmp_manual}
\end{figure*}

% by using a DJI Phantom 4 RTK, which is a single-camera drone with a focal length ranged from 8.8 to 24mm.

\subsection{Comparison with commercial software}
First, we compare our plane-based texture mapping results with  dense textured mesh reconstructed by the commercial software RealityCapture (RC) on scene Polytech. In detail, RC generates texture maps for reconstructed dense triangular facets while our method produces one complete texture map for each planar shape of the simplified coarse model. As illustrated in Fig.~\ref{fig:cmp_rc}, our plane-based method outputs more photo-realistic texture maps than RC on planar region. This phenomenon comes from two aspects. First, simplified models are composed by planar shapes, where the local homography perfectly holds between different views in each planar region. However, the distribution of clutter triangular facets of dense mesh destroys this local homography which causes the distortion of textures. Second, several input images are taken from a large distance by a drone and some small planar structures are not well reconstructed in the dense mesh, this would leads to a wrong UV mapping for these parts. However, our planar-based method performs on simplified mesh where important planar structures are well inherited.


\begin{figure*}[tp]
    \centering
    \includegraphics[width=\textwidth]{figs/compare.png}
    \caption{Visual comparison against LTBC~\cite{waechter2014let} and RC on three scenes with sharp texture details, where the detailed comparisons are shown in the zoomed-in insets.}
    \label{fig:cmp_noManual}
\end{figure*}

\begin{figure*}[tp]
    \centering
    \includegraphics[width=\textwidth]{figs/wudonglou.png}
    \caption{Visual comparison against LTBC~\cite{waechter2014let} and RC on more challenging scene Sunshine Plaza, where the detailed comparisons are shown in the zoomed-in insets.}
    \label{fig:wudonglou}
\end{figure*}

\subsection{Comparison with human-expert}
Next, we invite a professional human-expert to manually generate texture maps for simplified coarse models. Without any prior knowledge and pre-training, the human-expert employ a similar pattern involved in our method. First, he manually selects the boundary polygons for each planar shape and performs UV mapping to project 3D polygons to 2D space. Next, he carefully picks a set of visible views and clips the visible patches of current plane form each view. Finally, he transforms all the clipped patches to 2D space and merges them to align the boundary of polygons. The whole procedure usually costs about dozens of hours to texture a piecewise-planar buildings composed by one hundred planes reconstructed from few hundreds of high-resolution images. From Table~\ref{tab:cmp-time}, the simplified model occupies less memory than dense triangular mesh by five orders of magnitude. 

Fig.~\ref{fig:cmp_manual} exhibits the qualitative comparison between our full-automatic method and the above human-expert manual texturing mechanism. To explicitly illustrate the performance of two methods with respect to real scene, we also present the dense textured mesh reconstructed by RC. As shown in Fig~\ref{fig:cmp_manual}, both plane-based methods produce more photo-realistic texture meshes than RC. Moreover, manually texturing method sometimes miss-aligns line-segments in adjacent patches and collapses the global geometry features, while our method preserves the straightness and completeness of global lines. Another interesting point is that while handling invisible regions, human-expert usually selects similar texture patches from other public sources to complete the holes. However, our texture optimization operators can roughly inpaint these regions by propagating geometry regularity from visible part. Note that it takes 0.41h and 0.84h for our algorithm to perform the whole pipeline on scene Mobile and Hitech respectively, while human-expert spends 9h and 26h in manual texturing two models. 

\subsection{Comparison with texture generation methods}

%\noindent\textbf{Comparison on texture generation.} 
Besides, we also evaluate the quality of our generated texture maps by comparing against a popular and competitive texturing generation framework (\emph{Let There Be Color} (LTBC)~\cite{waechter2014let}).

 Fig.~\ref{fig:cmp_noManual} shows the qualitative results of two methods on three simplified coarse models with sharp texture details rendered from two view directions. Dense textured mesh returned by RC are also exhibited as reference results to measure the perceptive distance from textured models of two methods to real scenes. To be precise, LTBC selects the most suitable view for each facet and by solving a Markov Random Field formulation and adjust the pixels values along the boundary edges of adjacent patches to alleviate the seams. This strategy fails to texture large facet in case of there does not exist any camera view that can observe the whole region of the facet. Thus, for a fair comparison, we subdivide the simplified coarse model and perform LTBC to generate texture maps for the corresponding subdivided mesh.
%In the dense mesh of RC, a large-scale plane is usually represented by too many small triangular facets, resulting in inconsistent and cluttered textures between adjacent facets due to the camera misalignment and 3D reconstruction inaccuracies, as illustrated in Fig.~\ref{fig:cmp_manual}. 
%As a projection-based approach,~\cite{waechter2014let} selects an optimal view to texture each facet by solving a Markov Random Field formulation to alleviate the seams between adjacent patches. 
From Fig.~\ref{fig:cmp_noManual}, LTBC is not able to produce satisfactory results for large-scale invisible planar structure resulting in blurring and ghosting artifacts. However, our method can handle large unobserved region by propagating geometry regularity extracted from visible region nearby. Moreover, due to the lack of explicit constraints on the linear features of buildings, the texture generated by LTBC destroys these geometric structures, making it suffer from seriously distortion effects.  %and the mapping results are seriously distorted. 
In contrast, our image stitching mechanism succeeds in preserving the straightness and completeness of the line segments by constructing an adaptive mesh taking the original geometric primitives as constraints.
Next, large duplicate texture patterns are also well kept in our results. This is mainly because that we select a minimum subset of camera views for each planar shape instead of each facet. This strategy guarantees that each selected view is used to texture current plane as much as possible.
Finally, from the visual results we can see that the textures generated by our approach are very closer to real scenes and contain rarely blurring and seaming artifacts resulting from inaccurate camera parameters. %original input images

\begin{table}[!t]
    \centering
	\caption{The performance statistics of RC, LTBC~\cite{waechter2014let} and our algorithm.}  
	\resizebox{\columnwidth}{!}{
		%\begin{center}
			%\small
			\begin{tabular}{c c c c c c}
			\midrule[1pt]
			Scenes &   View Num. & Method  & Facet Num. & Model (Mb) & Texture (Mb) \\
			\midrule
			\multirow{3}{*}{Polytech}&  \multirow{3}{*}{908}      & RC          & 10,000,000     & 1440     & 108       \\
			                         &                            & LTBC        & 55,738         & 4.45     & 361      \\
                                     &                            & Ours        & 332            & 0.03     & 151      \\ \hline 
                                     
            \multirow{3}{*}{Mobile}  &  \multirow{3}{*}{468}      & RC          & 15,193,795     & 2160     & 143   \\
			                         &                            & LTBC        & 167488         & 15.60    & 107      \\
                                     &                            & Ours        & 70             & 0.01     & 69     \\ \hline
                                     
            \multirow{3}{*}{Hitech}  &  \multirow{3}{*}{308}      & RC          & 2,000,000      & 285      & 239        \\
			                         &                            & LTBC        & 179726         & 16.10    & 204       \\
                                     &                            & Ours        & 796            & 0.04     & 54      \\ \hline
                                     
            \multirow{3}{*}{Library} &  \multirow{3}{*}{970}      & RC          & 4,000,000      & 433      & 86         \\
			                         &                            & LTBC        & 90,098         & 9.18     & 264      \\
                                     &                            & Ours        & 207            & 0.01     & 53        \\ \hline
            
            \multirow{3}{*}{AntSci} &  \multirow{3}{*}{949}       & RC          & 8,278,218      & 980      & 360         \\
			                         &                            & LTBC        & 66,938         & 6.00     & 251      \\
                                     &                            & Ours        & 608            & 0.02     & 176        \\ \hline
            
            \multirow{3}{*}{Hall} &  \multirow{3}{*}{520}         & RC          & 2,999,999      & 383      & 230         \\
			                         &                            & LTBC        & 156,006        & 14.50    & 326      \\
                                     &                            & Ours        & 876            & 0.06     & 145        \\\hline
            
            \multirow{3}{*}{Sunshine Plaza} &  \multirow{3}{*}{945}      & RC          & 3,000,000      & 432      & 107    \\
			                         &                                   & LTBC        & 356,129        & 34.80    & 1120      \\
                                     &                                   & Ours        & 2,446          & 0.19     & 425        \\
			\midrule[1pt]
		\end{tabular}
		%\end{center}
 	}
\label{tab:cmp-time}
\end{table}

% \begin{table}[!t]%
% 	\caption{The performance statistics of RC, LTBC~\cite{waechter2014let} and our algorithm. LTBC\_c and LTBC\_s represent that we apply~\cite{waechter2014let} to texture the coarse mesh and a corresponding subdivided mesh, respectively.} 
% 	\label{tab:cmp-time}
% 	%\begin{minipage}{\linewidth}
% 	\vspace{-3mm}
% 	\resizebox{\linewidth}{!}{%
% 		\begin{center}
% 			\small
% 			\begin{tabular}{c c c c c c c}
% 			\midrule[1pt]
% 			\multirow{1}{*}{Scenes} & \multirow{1}{*}{Method} & Source View & View Size (Mb) & Model Facet & Model Size (Mb) & Texture Size (Mb)\\
% 			\midrule
% 			\multirow{4}{*}{Polytech}   & RC        & 908   & 6610   & 10,000,000     & 1440     & 108       \\
% 			\multicolumn{1}{c}{}        & LTBC      & 908   & 6610   & 55,738         & 4.45     & 361      \\
%             \multicolumn{1}{c}{}        & Ours      & 908   & 6610   & 332            & 0.03     & 151      \\ \hline 
            
%             \multirow{4}{*}{Mobile}     & RC        & 468   & 3400   & 15,193,795     & 2160     & 143   \\
% 			\multicolumn{1}{c}{}        & LTBC      & 468   & 3400   & 167488         & 15.60    & 107      \\
%             \multicolumn{1}{c}{}        & Ours      & 468   & 3400   & 70             & 0.01     & 69     \\ \hline
            
%             \multirow{4}{*}{Hitech}     & RC        & 308   & 2460   & 2,000,000      & 285      & 239        \\
% 			\multicolumn{1}{c}{}        & LTBC      & 308   & 2460   & 179726         & 16.10    & 204       \\
%             \multicolumn{1}{c}{}        & Ours      & 308   & 2460   & 796            & 0.04     & 54      \\ \hline
            
%             \multirow{4}{*}{Library}    & RC        & 970   & 7910   & 4,000,000      & 433      & 86         \\
% 			\multicolumn{1}{c}{}        & LTBC      & 970   & 7910   & 90,098         & 9.18     & 264      \\
%             \multicolumn{1}{c}{}        & Ours      & 970   & 7910   & 207            & 0.01     & 53        \\
            
% 			\midrule[1pt]
% 		\end{tabular}
% 		\end{center}
% 	    %\end{minipage}
% 	    \vspace{-5mm}
% 	}
% \end{table}%

Moreover, Fig.~\ref{fig:wudonglou} exhibits the visual texturing results on more challenging scene, which further demonstrates that our algorithm is able to produce high-fidelity textures with minimal artifacts. Table~\ref{tab:cmp-time} reports the scene information and performance statistics of different methods. Comparing to other methods, our approach is able to texture extremely coarse models (see the number of facets) while achieving minimal storage overhead.   
%Although~\cite{waechter2014let} perform best in terms of running time, their method cannot address the misalignments of geometric features such as line segments. Our method is fully automatic and considerably faster comparing to RC and manual texturing. Moreover, our implementation is not optimized yet, of which many steps can be parallelized. Thus, in future we could implement it on GPU for further acceleration \jwc{please check}.


% \begin{figure}[!thp]
%     \centering
%     \includegraphics[width=\linewidth]{figs/placeholder}
%     \vspace{-0.5cm}
%     \caption{Comparison on image stitching.}
%     \label{fig:cmp_stitching}
% \end{figure}

%- compare our methods with manual method and facet-based method (let there be color) by both qualitative and quantitative results

%\noindent\textbf{Comparison on image stitching.}
%Next, to demonstrate the performance of our line-preserving image stitching mechanism guided by adaptive-mesh data structure, we compare with two state-of-the-art image stitching approaches, including~\cite{liao2019single} and~\cite{jia2021leveraging}, both of which apply an uniform grid to warp the images to maintain the global geometry features. In order to quantify the stitching performance on linear structures, we adopt the metrics introduced by~\cite{jia2021leveraging} to measure the distance of matched lines and the discrepancy in the direction of matched lines. Specifically, the distance term $E_{dis}$ represents the average distance between two warped endpoints and the matching line pairs, which is described as:
%\begin{equation}
%E_{dis} = \sqrt{\frac{1}{L}\sum_{j=1}^{i=L}\|\frac{dis(l_{j}^{'},p_{s}^{j}) + dis(l_{j}^{'},p_{e}^{j})}{2}\|^2},
%\end{equation}
%where $l_{j}^{'}$ represents the $j^{th}$ matching line of the reference image, $p_{s}^{j}$ and $p_{e}^{j}$ are two endpoints of the $j^{th}$ matching line in target image.
%The direction term $E_{dir}$ computes the direction difference between the warped line and the matching line, which is defined as: 
%\begin{equation}
%E_{dir} = \sqrt{\frac{1}{L}\sum_{j=1}^{i=L}\|sin(\theta)\|^2},
%\end{equation}
%where $\theta$ denotes the angle between the warped line and the matching line. 

\subsection{Ablation Study}
%\noindent\textbf{Comparison on image stitching.}
Finally, we conduct an ablation experiment to validate the effectiveness of our designed adaptive mesh data-structure for preserving line structures. To this end, in the image stitching stage, instead of using adaptive mesh to warp the texture patch, we directly blend all the texture patches one by one for each plane. 
Fig.~\ref{fig:ablation} shows the stitching results with and without adaptive mesh deformation. 
The comparison demonstrates that by using the adaptive mesh to locally deform the image, we are able to explicitly maintain the alignment of line-segments in the overlapping areas of different texture patches. 

Moreover, we also compare with two state-of-the-art image stitching approaches on scene Polytech, Mobile and Hitech, including~\cite{liao2019single} and~\cite{jia2021leveraging}, both of which apply an uniform grid to warp the images to maintain the global geometry features. In order to quantify the stitching performance on linear structures, we adopt the metrics introduced by~\cite{jia2021leveraging} to measure the distance of matched lines and the discrepancy in the direction of matched lines. Specifically, the distance term $E_{dis}$ represents the average distance between two warped endpoints and the matching line pairs, which is described as:
\begin{equation}
E_{dis} = \sqrt{\frac{1}{L}\sum_{j=1}^{i=L}\|\frac{dis(l_{j}^{'},p_{s}^{j}) + dis(l_{j}^{'},p_{e}^{j})}{2}\|^2},
\end{equation}
where $l_{j}^{'}$ represents the $j^{th}$ matching line of the reference image, $p_{s}^{j}$ and $p_{e}^{j}$ are two endpoints of the $j^{th}$ matching line in target image.
The direction term $E_{dir}$ computes the direction difference between the warped line and the matching line, which is defined as: 
\begin{equation}
E_{dir} = \sqrt{\frac{1}{L}\sum_{j=1}^{i=L}\|sin(\theta)\|^2},
\end{equation}
where $\theta$ denotes the angle between the warped line and the matching line.

\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/ablation_adatpive.png}
    \caption{Ablation study of adaptive mesh data-structure on scene Polytech, Mobile and Hitech. Left: with adaptive mesh; Right: without adaptive mesh.}
    \label{fig:ablation}
\end{figure}

\begin{table}[tp]%
	\caption{Quantitative comparison on stitching performance of different image stitching methods.} 
	\label{tab:cmp-stitching}
	%\begin{minipage}{\linewidth}
%	\vspace{-3mm}
	%\resizebox{\linewidth}{!}{%
		\begin{center}
	%		\small
			\begin{tabular}{c c c c}
			\midrule[1pt]
			\multirow{1}{*}{Scenes} & \multirow{1}{*}{Methods} & $E_{dis} \downarrow$ & $E_{dir} \downarrow$ \\
			\midrule
			\multirow{3}{*}{Polytech}   & ~\cite{liao2019single}        & 4.07870   & 0.01715              \\
			\multicolumn{1}{c}{}        & ~\cite{jia2021leveraging}     & \textbf{2.99699}   & 0.02584               \\
            \multicolumn{1}{c}{}        & Ours                          & 3.62430   & \textbf{0.01459}                  \\ \hline 
            \multirow{3}{*}{Mobile}     & ~\cite{liao2019single}      & 1.04808   & 0.00952              \\
			\multicolumn{1}{c}{}        & ~\cite{jia2021leveraging}   & 1.35084   & 0.01209               \\
            \multicolumn{1}{c}{}        & Ours      & \textbf{0.37151}   & \textbf{0.00102}       \\ \hline  
            \multirow{3}{*}{Hitech}   & ~\cite{liao2019single}      & 1.06089   & 0.01142              \\
			\multicolumn{1}{c}{}        & ~\cite{jia2021leveraging}   & 2.60402   & 0.01350               \\
            \multicolumn{1}{c}{}        & Ours      & \textbf{0.96814}   & \textbf{0.00568}                \\ 
			\midrule[1pt]
		\end{tabular}
		\end{center}
\end{table}%

% Fig.~\ref{fig:cmp_stitching} gives the visual comparison of different stitching methods, where from \jw{three} scenes we select representative planes with high-quality textures and a large number of matching lines for evaluation. 
From three scenes we choose a set of representative planes with high-quality textures and a large number of matching lines for quantitative comparison of different stitching methods. 
Table~\ref{tab:cmp-stitching} reports the performance for preservation of linear structures using above two measures. 
From the comparison, we can see that our method outperforms~\cite{liao2019single} and~\cite{jia2021leveraging} in distance and differences of angles on scene Mobile and Hitech. This improvement mainly comes from the property of our adaptive mesh which takes geometric primitives as constraints and controls the deformation of each line-segment independently comparing against the grid mesh involved in ~\cite{liao2019single} and~\cite{jia2021leveraging}.

% \subsection{Limitations}



% These methods can generate texture maps with lots of
% details. However, these methods cannot perfectly address the misalignments of
% images resulting in blurring and ghosting artifacts. Lempitsky and Ivanov [15]
% diminish visible seams by performing a global color adjustment following with
% Poisson editing [21]. However, blurring and ghosting artifacts around seams may
% still occur due to noisy input data. Other approaches are proposed to gener-
% ate seamless texture maps using geometry information. For example, Barnes et
% al. [3] provide an interactive method to manually correct misaligned errors be-
% tween the geometry model and images, which is not suitable for E-Commerce
% applications. Bi et al. [5] propose a patch-based optimization that incorporates
% geometry information. Their method estimates the bidirectional similarity of dif-
% ferent images, which suffers from high computational cost. 


% RC would produce distorted and misaligned artifacts due to the camera misalignment and 3D reconstruction inaccuracies.

% However, this method is not able to produce satisfactory results in this case, since they assign inconsistent textures to some of the adjacent faces because of significant inaccuracies. 

% Furthermore, they all fail to align large-scale geometric features, resulting in obvious seams in the generated texture maps

% Figure 5 shows the resulting image optimized with our approach in comparison to a naive L1 loss

% Waechter et al. [2014] select one view per
% face by solving an optimization system to hide the seams between
% adjacent faces. However, their method is not able to produce satisfactory results in this case, since they assign inconsistent textures to
% some of the adjacent faces because of significant inaccuracies. Note
% the tearing artifacts at the top inset and the distorted bear face at
% the bottom inset. Moreover, the local warping in Zhou and Koltun’s
% approach [2014] is not able to correct significant misalignment in
% this case, caused by inaccurate geometry (see Fig. 10). Therefore,
% their results suffer from ghosting and blurring artifacts. Our method
% synthesizes aligned target images and is able to produce high-quality
% texture maps with minimal artifacts.

==> src/backup/old-src/06-future.tex <==
%\section{Conclusion}
\section{Conclusion and Future Work}

In this work, we proposed a plane-based texture generation method to produce texture maps for objects composed of piecewise-planar shapes. Our main technical contributions consist in i) employing a submodular formulation to select a minimum set of views that are most suitable for texturing each planar shape, and ii) stitching the selected views to an enlarged texture map by detecting and preserving the significant linear geometric primitives relying on an adaptive-mesh data structure. Experimental results show that our algorithm outperforms state-of-the-art facet-based texture generation methods in the quality of texture maps. %Moreover, our method produces production-level texture maps in a computational time two orders of magnitudes smaller than an as human-expert \fh{[FH: please check]}.

\noindent\textbf{Limitations and future work.} Our algorithm still has several limitations. First, planar shapes with a large part of itself is not observed by any camera views can not be handled in our current implementation. Second, the visible misalignment between the planar shape and camera views in case of large geometry displacement of original mesh is not well studied in our system. Third, our plane-based texture generation method process each planar shape independently, which does not take their mutual relationship into consideration to improve the texture maps in a global manner. We will incorporate these issues in our future pipeline.
